ASV: Accelerated Stereo Vision System

Estimating depth from stereo vision cameras, i.e., "depth from stereo", is critical to emerging intelligent applications deployed in energy- and performance-constrained devices, such as augmented reality headsets and mobile autonomous robots. While existing stereo vision systems make trade-offs between accuracy, performance and energy-efficiency, we describe ASV, an accelerated stereo vision system that simultaneously improves both performance and energy-efficiency while achieving high accuracy. The key to ASV is to exploit unique characteristics inherent to stereo vision, and apply stereo-specific optimizations, both algorithmically and computationally. We make two contributions. Firstly, we propose a new stereo algorithm, invariant-based stereo matching (ISM), that achieves significant speedup while retaining high accuracy. The algorithm combines classic "hand-crafted" stereo algorithms with recent developments in Deep Neural Networks (DNNs), by leveraging the correspondence invariant unique to stereo vision systems. Secondly, we observe that the bottleneck of the ISM algorithm is the DNN inference, and in particular the deconvolution operations that introduce massive compute-inefficiencies. We propose a set of software optimizations that mitigate these inefficiencies. We show that with less than 0.5% hardware area overhead, these algorithmic and computational optimizations can be effectively integrated within a conventional DNN accelerator. Overall, ASV achieves 5x speedup and 85% energy saving with 0.02% accuracy loss compared to today DNN-based stereo vision systems.

==> ASV_ Accelerated Stereo Vision System/abstract.tex <==
\begin{abstract}

Estimating depth from stereo vision cameras, i.e., "depth from stereo", is critical to emerging intelligent applications deployed in energy- and performance-constrained devices, such as augmented reality headsets and mobile autonomous robots. 
While existing stereo vision systems make trade-offs between accuracy, performance and energy-efficiency, we describe \proj, an accelerated stereo vision system that simultaneously improves both performance and energy-efficiency while achieving high accuracy.

%To design a real-time stereo vision, it is necessary to understand and leverage its unique characteristics which current designs lack of. In this work, we proposed \proj, which combined the features in both state-of-the-art DNN and classic algorithms. 

The key to \proj is to exploit unique characteristics inherent to stereo vision, and apply stereo-specific optimizations, both algorithmically and computationally. We make two contributions. Firstly, we propose a new stereo algorithm, \textit{invariant-based stereo matching} (ISM), that achieves significant speedup while retaining high accuracy. The algorithm combines classic ``hand-crafted'' stereo algorithms with recent developments in Deep Neural Networks (DNNs), by leveraging the \textit{correspondence invariant} unique to stereo vision systems. 
Secondly, we observe that the bottleneck of the ISM algorithm is the DNN inference, and in particular the \textit{deconvolution} operations that introduce massive compute-inefficiencies. 
We propose a set of software optimizations that mitigate these inefficiencies. 
We show that with less than 0.5\% hardware area overhead, these algorithmic and computational optimizations can be effectively integrated within a conventional DNN accelerator. Overall, \proj achieves 5$\times$ speedup and 85\% energy saving with 0.02\% accuracy loss compared to today's DNN-based stereo vision systems.

\end{abstract}

==> ASV_ Accelerated Stereo Vision System/algorithm.tex <==
\section{Invariant-based Stereo Matching}
\label{sec:algo}

This section introduces our new \textit{invariant-based stereo matching algorithm} (ISM). 
The key idea of ISM is to exploit the \textit{correspondence invariant} between the stereo images over time. 
After introducing the high-level concept (\Sect{sec:algo:idea}), we then describe the detailed algorithm (\Sect{sec:algo:details}), and discuss important algorithmic design decisions (\Sect{sec:algo:design}). We make the implementation of ISM available at: \url{https://github.com/horizon-research/ism-algorithm}.

%show the details of our integrated algorithm and how our algorithm explores some unique characteristics in stereo vision. We show the overview of our integrated algorithm in  and detailed procedure in . The implementation details are shown in \Sect{subsec:algorithm_implementation}.

\subsection{Overview}
\label{sec:algo:idea}

%Despite the high performance of DNN algorithm, its high computation latency often prevent applications achieving a real-time response on a commodity mobile device. To solve this dilemma, an ideal algorithm should reduce the response latency meanwhile maintain the DNN algorithm-level accuracy. Being inspired by the idea of triangulation, we propose this integrated algorithm to solve this issue.

Stereo matching produces a disparity map~(\Fig{fig:dispmap}), from which depth information is easily obtained through triangulation~(\Fig{fig:triangulation}).
Classic stereo matching algorithms generate the disparity map by matching pixels/features in the left (reference) frame with pixels/features in the right (matching) frame, typically by searching in a finite window. 
However, the accuracy of search-based algorithms is sensitive to the heuristics used in the search, such as feature selection, search window size, matching criterion, etc. 
In contrast, DNN approaches largely avoid heuristics and instead directly learn the matching pairs.
Unfortunately, DNNs come at the cost of a massive increase in compute requirement.

Instead of the binary choice between DNNs and conventional search-based algorithms, we use DNNs to \textit{guide} the search process of classic methods. 
The key observation is that two matched pixels, one from the left image and the other from the right image, correspond to the same point in the physical world. 
While the locations of the two pixels move from frame to frame, they are always projections of the same scene point, and therefore are always a matched pair in any frame. 
In other words, the geometric correspondence relationship between two matched pixels is invariant.

Our new stereo matching algorithm, ISM, exploits this \textit{correspondence invariant} by operating in two modes. 
It obtains stereo correspondences on ``key frames'' through accurate but compute-intensive DNNs. 
The correspondences are then propagated to subsequent non-key frames as good initial guesses to guide the cheaper search-based methods. By combining learnt correspondences with search-based methods that explicitly model the physical world, ISM reduces the total compute cost while retaining DNN-like accuracy.
%Since the search-based methods are much cheaper than CNNs, the stereo correspondences in the current frame are obtained much more efficiently.

%Once we derive the accurate matching pixels in one frame (e.g., through DNNs), this invariant allows us to propagate the matching information to subsequent frames. This matching information provides critical searching hints to guide the classic algorithms with high accuracy.

%In a typical DNN pipeline, the disparity map is produced by a DNN inference. Then, the disparity map is used to compute the depth map using triangulation. This procedure repeats for every frame pair, as shown on the left of \Fig{fig:motion_algorithm}. 

\subsection{Algorithm}
\label{sec:algo:details}

We illustrate ISM in \Fig{fig:motion_algorithm}. 
ISM consists of four main components. 
ISM runs DNN inferences (\circled{white}{1}) on key frames to obtain pixel correspondences, which are used to guide feature matching on non-key frames (\circled{white}{2}, \circled{white}{3}, and \circled{white}{4}).

%Instead of discarding the disparity immediately after computing the depth map, we take a full advantage of the disparity map from the current frame pair and use it to extrapolate the disparity map of new coming frame pairs. The extrapolation is proceeded as follows. From current disparity map, we can closely match two pixels on the left and the right image. By using some algorithm to compute the motion of current and next frame pair, we are able to locate each pixel pair in the next frame pair. By knowing the exact location of each pixel pair in the next frames, we are able to extrapolate the disparity map of the next frames without going through DNN pipeline, as shown on the right of \Fig{fig:motion_algorithm}. Next, we show the details of extrapolation algorithm.

%To better distinguish the disparity map from different methods, we named the disparity map from DNN inference I-map and one from extrapolation algorithm E-map. The detail of our algorithm proceeds as follows.

\paragraph{\circled{white}{1} DNN Inference} Assuming the left and right frames at timestep $t$ are regarded as key frames, ISM performs DNN inference to generate a disparity map for the left image, in which each pixel value represents the disparity (i.e., $Z$ in \Fig{fig:triangulation}) of each pixel in the left frame. 
In conventional DNN approaches, this disparity map is used only for triangulation (not shown in the figure) to estimate depth, and is discarded after the depth map is generated.

\paragraph{\circled{white}{2} Reconstruct Correspondences} Instead of discarding the disparity map, ISM uses it to identify the correspondences in the left and right frames. 
As per the definition of disparity (\Equ{eq:dispdef}), every <$x_{t}, y_{t}$> pixel in the disparity map with the value $D_{t}^{\text{<}x, y\text{>}}$ indicates that the <$x_{t}, y_{t}$> pixel in the left frame ($P_{t}^{L}$) and the <$x_{t} + D_{t}^{\text{<}x, y\text{>}}, y_{t}$> pixel in the right frame ($P_{t}^{R}$) form a correspondence pair. 
By iterating through all the pixels in the disparity map, ISM identifies all the correspondence pairs in the left and right frames at timestep $t$.
% Each correspondence pair (e.g., $P_{t}^{l}$ and $P_{t}^{r}$) are projected from the same point in the physical world.

%First, we reserve the previous I-map, $ Disp^{(t)} $, from DNN inference at time $t$. By using $ Disp^{(t)} $, we can pair any pixel in $ L^{(t)} $ with a pixel in $ R^{(t)} $. As \Fig{fig:motion_algorithm} shows, two small patches are paired from $ L^{(t)} $ and $ R^{(t)} $ at time $t$.

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{motion_algorithm}
\caption{The ISM algorithm obtains correspondences in key frames using DNNs, and propagates the correspondences to non-key frames to guide the cheap correspondence search. Time progresses from top to bottom in the figure.}
%\vspace{-10pt}
\label{fig:motion_algorithm}
\end{figure}

\paragraph{\circled{white}{3} Propagate Correspondences} A new pair of frames arrives at the next timestep $(t+1)$. 
ISM exploits a well-known observation that pixels in consecutive video frames are highly-correlated in time. 
For instance, $P_{t}^{L}$ has moved to $P_{t+1}^{L}$, and $P_{t}^{R}$ has moved to $P_{t+1}^{R}$. Critically, since $P_{t}^{L}$ and $P_{t}^{R}$ are a correspondence pair projected from a scene point, $P_{t+1}^{L}$ and $P_{t+1}^{R}$ must correspond to the same point, and hence highly likely to also be a correspondence pair at timestep $(t+1)$.
%In other words, although pixels in a matched pair move across frames, their correspondence does not change, hence the invariant.

The exact coordinates of $P_{t+1}^{L}$ and $P_{t+1}^{R}$ can be obtained through a \textit{motion estimation} (ME) algorithm. For each pixel in the left (right) frame, the ME algorithm generates a motion vector $\Delta P^{L}_{(t+1, t)}$ ($\Delta P^{R}_{(t+1, t)}$), representing the displacement between the pixel in frame $t$ and frame $(t+1)$. Thus:
%%$$ \Delta L_{(t+1, t)} = MotionEstimation(L_{t+1}, L_{t}) $$
%%$$ \Delta R_{(t+1, t)} = MotionEstimation(R_{t+1}, R_{t}) $$
% $$ \text{<}x^{l}_{t+1}, y^{l}_{t+1}\text{>}~=~\text{<}x^{l}_{t}, y^{l}_{t}\text{>}~+~\Delta L_{(t+1, t)} $$
% $$ \text{<}x^{r}_{t+1}, y^{r}_{t+1}\text{>}~=~\text{<}x^{r}_{t}, y^{r}_{t}\text{>}~+~\Delta R_{(t+1, t)} $$
$$ P_{t+1}^{L}~=~P_{t}^{L}~+~\Delta P
^{L}_{(t+1, t)} $$
$$ P_{t+1}^{R}~=~P_{t+1}^{R}~+~\Delta P^{R}_{(t+1, t)} $$

\paragraph{\circled{white}{4} Refine Correspondences} Given the correspondence pairs (e.g., $P_{t+1}^{L}$ and $P_{t+1}^{R}$) at timestep $(t+1)$, ISM then calculates the disparity map at $(t+1)$. 
If the motion estimation from $t$ to $(t+1)$ is precise, the propagated correspondence pairs at $(t+1)$ are also precise. 
Accordingly, the disparity map could be simply obtained by calculating the horizontal offsets between all the correspondence pairs. 
For instance, given the correspondence pair $P_{t+1}^{L}$ and $P_{t+1}^{R}$, the disparity at <$x^{l}_{t+1}, y^{l}_{t+1}$> in the disparity map would be $ x^{r}_{t+1} - x^{l}_{t+1}$.

In reality, motion estimation is imperfect due to various visual artifacts such as occlusion and fast motion~\cite{liu1998accuracy}. 
Thus, the correspondences propagated from $t$ are a noisy estimate of the true correspondences at $(t+1)$. 
To further refine the estimate of $(t+1)$ in ISM, we use classic \textit{correspondence search}, and initializes the search window with the propagated correspondences. 
This allows ISM to avoid compute-intensive DNNs on non-key frames without sacrificing accuracy.

%Specifically, ISM resorts to classic search-based algorithms to calculate the matched pairs at $(t+1)$, from which disparity can then be obtained.

%After locating each pair of pixel in $ L^{(t+1)} $ and $ R^{(t+1)} $, we can simply compute the distance between $ L^{(t+1)} $ and $ R^{(t+1)} $ in x-axial to construct the disparity map, $ Disp(t+1)$.

%$$Disp^{(t+1)}(x_l', y_l') = R^{(t+1)}(x_r', y_r') - L^{(t+1)}(x_l', y_l') $$

\subsection{Algorithmic Design Decisions}
\label{sec:algo:design}

Computing non-key frames requires reconstructing, propagating, and refining correspondences. 
Reconstructing correspondences has little overhead. 
The cost of propagating correspondences is dominated by motion estimation, and the cost of refining correspondences is dominated by the correspondence search. 
Thus, we must carefully choose the motion estimation and correspondence search algorithms such that the compute cost is much lower than DNNs with little accuracy loss. We discuss algorithmic choices below.

\paragraph{Motion Estimation} The literature is rich with motion estimation algorithms, which differ in the coverage and densities of estimated motion. 
The disparity map in stereo matching should ideally be calculated on a per-pixel basis across the frame, so as to enable fine-grained depth estimation. 
This requirement rules out many classic motion estimation algorithms such as block matching (BM)~\cite{bmsurvey}, and sparse optical flow~\cite{lucas1981iterative, horn1981determining}. 
BM estimates motion at the granularity of a block of pixels, and thus does not provide the pixel-level motion that stereo vision requires. Sparse optical flow algorithms such as Lucas-Kanade~\cite{lucas1981iterative} and Horn-Schunck~\cite{horn1981determining} only provide pixel-level motion for feature points such as corners, and do not cover all the frame pixels.

Instead, we use a \textit{dense optical flow} algorithm, specifically the Farneback algorithm~\cite{farneback2003two, farneback2002polynomial}, for motion estimation. Farneback generates per-pixel motion for all the pixels, and is computationally efficient. 99\% of the compute in Farneback is due to three operations: Gaussian blur, ``Compute Flow'', and ``Matrix Update''. Gaussian blur is inherently a convolution operation that convolves a Guassian kernel (2D matrix) with the image. The latter two are point-wise operations that resemble the activation function in DNNs. Thus, motion estimation in the ISM algorithm can be computed using a DNN accelerator to simplify the hardware design.

\paragraph{Correspondence Search} ISM performs correspondence search to refine the initial correspondence estimation propagated through motion. Correspondence search algorithms have been well-studied in the classic computer vision literature~\cite{stereo2002scharstein, stereo2003Brown}, and generally fall into two categories: local methods and global methods. At the cost of higher compute demand, global methods provide higher accuracy by minimizing the pixel motion inconsistencies across the entire image. However, with the initial correspondences propagated through key-frames, we find that local methods suffice.

In particular, we leverage the block matching algorithm~\cite{bmsurvey} for local correspondence search. For each pixel in the left image (e.g., $P_{t+1}^{L}$ in \Fig{fig:motion_algorithm}), ISM uses the block of pixels surrounding it to search in a 1D window in the right image in order to find the closest match. The search window is centered around the initial correspondence estimation (e.g., $P_{t+1}^{R}$ in \Fig{fig:motion_algorithm}). We use the sum of absolute differences (SAD) cost function. The horizontal offset between the two matched blocks is the disparity for $P_{t+1}^{L}$.

Similar to optical flow, the block matching algorithm has a ``convolution-like'' structure~\cite{qadeer2013convolution}; the block in the left image is equivalent to a kernel, and the search window in the right image is equivalent to the input image. 
The only difference is that block matching computes the SAD between the input feature map and the kernel ($\sum^{N}_{i=1} |a_i - b_i|$) as opposed to the dot product in canonical convolution ($\sum^{N}_{i=1} a_i b_i$). 
Thus, the correspondence search can share the same architecture as DNNs and optical flow.

\paragraph{Compute Cost} Due to our algorithmic choices, computation on non-key frames is much cheaper than key-frames. For instance, for a typical qHD frame (960 $\times$ 540), computating a non-key frame requires about 87 million operations while stereo DNN inference (key frame) requires about $10^2\times$--$10^4\times$ more arithmetic operations. 
Thus, ISM leads to significant performance and energy improvements by avoiding DNN inference altogether in non-key frames.

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{split_deconv.pdf}
%\vspace{-5pt}
\caption{Translating deconvolution into multiple convolutions. Standard deconvolution first upsamples the \textit{ifmap} before convolving with the kernel. Note that this example assumes the upsampled \textit{ifmap} is not further padded before the convolution, i.e., a $7 \times 7$ \textit{ifmap} results in a $5 \times 5$ \textit{ofmap}. Our translation algorithm holds regardless of padding.}
\label{fig:split_deconv}
\end{figure*}

%Specifically, we search a horizontal 1D search-window around $P_{t+1}^{R}$ and find the best match for $P_{t+1}^{L}$ to determine the disparity of $P_{t+1}^{L}$. In other words, the locations of $P_{t+1}^{L}$ and $P_{t+1}^{R}$ can be viewed as providing an initial guess as to where the matching pairs are, guiding the search process.





==> ASV_ Accelerated Stereo Vision System/background.tex <==
\section{Background}
\label{sec:bcg}

We first describe the scope of our work: vision-based systems that extract 3D information from 2D stereo images (\Sect{sec:bcg:depth}). 
We then introduce the necessary background of stereo vision algorithms, including both classic hand-crafted algorithms and contemporary stereo DNNs (\Sect{sec:bcg:sv}).

%In the following paragraphs, we briefly introduce these two key steps in stereo vision algorithms (\Sect{subsec:sv_bg}) and some necessary backgrounds of DNN (\Sect{subsec:cnn}). \Sect{subsec:tradeoff} shows the motivation of our framework.

\subsection{Depth Sensing}
\label{sec:bcg:depth}

There are two essential methods to extract depth information: passive sensing and active sensing. 
Passive sensing techniques observe the environment, primarily through cameras, and infer depth using computer vision algorithms. 
In contrast, active sensing techniques transmit signals and analyze the response to calculate depth; examples include structured light~\cite{wang20123d} and LiDAR~\cite{weitkamp2006lidar}.

This paper focuses on camera-based passive sensing. Compared to alternatives such as LiDAR, cameras are much cheaper and less bulky~\cite{camera_comparison}. As a result, camera-based depth sensing is widely adopted in systems such as autonomous vehicles and AR headsets. According to Allied Market Research, the adoption of stereo cameras is expected to grow 60.4\% by 2020~\cite{3dcammarket}. The recent industry trend of integrating dedicated stereo vision accelerators into mobile SoCs (e.g., Movidius~\cite{myriadx} and Nvidia~\cite{xaviersoc}) further underlines the significance of stereo vision for depth sensing.

\subsection{Depth From Stereo}
\label{sec:bcg:sv}

\begin{figure}[t]
%\vspace{-8pt}
\centering
\subfloat[\small{Triangulation.}]
{
  \includegraphics[trim=0 0 0 0, clip, height=1.65in]{triangulation}
  \label{fig:triangulation}
}
\subfloat[\small{Disparity Map.}]
{
  \includegraphics[trim=0 0 0 0, clip, height=1.65in]{dispmap}
  \label{fig:dispmap}
}
\caption{``Depth from stereo'' illustration: given an image pair, \textit{stereo matching} algorithms first generate the disparity map~\protect\subref{fig:dispmap}, from which depth is then calculated through \textit{triangulation}~\protect\subref{fig:triangulation}. Triangulation is computationally trivial; this paper focuses on optimizing stereo matching algorithms.}
\label{fig:sm}
%\vspace{-8pt}
\end{figure}

%Vision systems estimate the depth using two 2D images captured from two vantage points of the same scene, mimicking the biological stereopsis process. 
%The stereo image pair could either be taken from two cameras that are horizontally placed (binocular vision) or from one single camera that is in controlled motion (monocular vision)~\cite{MonoStereo2017, MonoOdometry2013}. 
%Our paper focuses on the fundamental principles of stereo vision, and is independent of how the stereo images are taken.

\paragraph{Triangulation} The key idea behind stereo depth estimation is that a single physical scene point projects to a unique pair of pixels, via two observing cameras; the horizontal displacement between the two pixels captured on the left and right image planes is inversely proportional to the distance of the point from the observer (i.e., the depth).~\Fig{fig:triangulation} illustrates this process, where the scene point is captured at position $x^l$ and $x^r$ on the left and right image planes, respectively. Using similar triangles, the depth $D$ is calculated by:
\begin{equation}
  \label{eq:triangulation}
  D = B f / Z,	
\end{equation}
\noindent where $f$ is the focal length of the cameras, $B$ is the distance between the two camera lenses, and $Z$ is the \textit{disparity} $x^r - x^l$, i.e., the horizontal displacement between the two corresponding pixels in the left and right images. This process is widely known as \textit{triangulation}~\cite{hartley2003multiple, szeliski2010computer}.

%\begin{equation}
%\frac{D}{D+f} = \frac{B}{B+Z}
%\end{equation}

%\textit{Disparity map} is a map that represents all the corresponding disparities of pixel pair. Most of stereo matching algorithms are aimed to compute disparity map first, and then use triangulation to compute depth map. The state-of-the-arts nowadays are using DNN algorithms.

%In order to compute a depth map of the current scene, there are two key steps: \textit{stereo matching} and \textit{triangulation}. Triangulation is computationally light and fast, the key in stereo vision is to improve the accuracy of stereo matching. Nowadays, many studies have used DNN to improve the accuracy on stereo vision.
%
%\paragraph{Triangulation} People found out to use s simple trick, \textit{triangulation}, to compute a depth map hundreds of years ago. \Fig{fig:triangulation} shows a schematic way to compute the depth of a object.


\paragraph{Stereo Matching and Disparity Map} Since both $B$ and $f$ are camera intrinsic parameters, the key to triangulation is to calculate the disparity $Z$. Given the left (reference) image and the right (matching) image, we must find the pixels in each image that are the projections of the same physical point, a process also known as \textit{stereo matching}. 
In the end, stereo matching generates a ``disparity map'', whose <$x, y$> coordinates are taken to be coincident with the pixel coordinates of the reference image.~\Fig{fig:dispmap} shows one such example, in which the correspondence between a pixel <$x^l, y^l$> in the left image and a pixel <$x^r, y^r$> in the right image is given by:
\begin{equation}
  \label{eq:dispdef}
  x^r = x^l + D^{\text{<}x^l, y^l\text{>}},~~~y^r = y^l,
\end{equation}
\noindent where D<$x^l, y^l$> denotes the pixel value at <$x^l, y^l$> in the disparity map. Note that the compute cost of triangulation is trivial (\Equ{eq:triangulation}), and thus we focus on stereo matching.

%, in which each pixel corresponds to the disparity value $Z$ of every pixel in the left image. The dual disparity map for the right image is omitted here as one disparity map is sufficient to calculate the depth.


Stereo matching algorithms consist of three stages~\cite{stereo2002scharstein, stereo2003Brown}: Feature Extraction (FE), Matching Optimization (MO), and Disparity Refinement (DR). 
Both conventional algorithms~\cite{stereo2002scharstein, stereo2003Brown, SGBM2008HH, StereoClass2008} and DNN-based algorithms~\cite{StereoClass2008, PSMNet2018, NvStereo2018, DispNet2015, GCNet2017} follow this processing pipeline, but differ in their implementations. 
Conventional methods extract hand-crafted features (e.g., SIFT~\cite{sift}, HOG~\cite{hog}, or plain pixel values) in the FE stage, search the feature space of both images to find the matching pixels in the MO stage, and improve the disparity resolution in the DR stage using techniques such as iterative gradient descent~\cite{tian1986algorithms}. DNNs, in contrast, implement each stage using a set of learnt parameters.
%, generally achieving higher accuracy while posing orders of magnitude higher compute demand.

\begin{figure}[t]
%\vspace{-2pt}
  \begin{minipage}[t]{0.45\columnwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, height=1.55in]{computation_cost}
    \caption{The arithmetic operation distribution of stereo matching DNNs.}
    \label{fig:cost_distribution}
  \end{minipage}
  \hspace{8pt}
  \begin{minipage}[t]{0.45\columnwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, height=1.55in]{sensitive-disp}
    \caption{Depth estimation accuracy is sensitive to stereo matching accuracy.}
    \label{fig:sensitive_disp}
  \end{minipage}
%\vspace{-10pt}
\end{figure}

\paragraph{Deconvolution in Stereo DNNs} Stereo matching DNNs implement FE and MO stages as convolution layers. The DR stage fundamentally requires \textit{deconvolution} (a.k.a. transposed convolution) layers~\cite{odena2016deconvolution}. Deconvolution layers generate large activation maps from small input feature maps, essentially up-sampling the input. The up-sampling in DR is critical to compensate the down-sampling in FE and MO that scale down the input images to extract high-level features.

To illustrate the importance of deconvolution in stereo vision,~\Fig{fig:cost_distribution} shows the time distribution of four state-of-the-art stereo matching DNNs across the three stages. The convolution and deconvolution layers combined account for over 99\% of the execution time, from which 38.2\% is attributed to the deconvolution layers.

\paragraph{High Accuracy Stereo Matching} Stereo matching is critical because it generates the disparity, from which depth is estimated (\Equ{eq:triangulation}). Using the industry-standard Bumblebee2 stereo camera~\cite{bumblebee2} as an example (B is \SI{120}{\milli\metre}, \textit{f} is \SI{2.5}{\milli\metre}, and pixel size is \SI{7.4}{\micro\metre}), \Fig{fig:sensitive_disp} shows how the depth estimation error ($y$-axis) varies with the disparity error in pixels ($x$-axis). Different curves correspond to objects at different distances. We find that even two tenths of a pixel error in stereo matching can result in a depth estimation error of 0.5m--5m, which could be catastrophic at the application level.

While existing stereo matching systems achieve high accuracy at the expense of high compute cost, \proj achieves DNN-level accuracy with significantly less compute.

%Some algorithms might skip one or two of these steps on the actual implementation. However, these steps consist the core in stereo vision algorithms. Even in recent years with the high popularity of DNN algorithms, those steps can still be reflected in DNN architectures~\cite{McCNN2015,NvStereo2018,GCNet2017,DispNet2015,PSMNet2018}, as we have shown in . 

%matching algorithms~\cite{} search the matching pixels via hand-crafted features extracted from both images. State-of-the-art methods use learnt features through DNNs~\cite{}, which achieve significantly higher accuracy at the expense of compute efficiency.

%\paragraph{Stereo Matching} Many stereo matching algorithms have been proposed in recent decades~\cite{stereo2002scharstein, stereo2003Brown, SGBM2008HH, StereoClass2008, PSMNet2018, NvStereo2018, DispNet2015, GCNet2017}.

%Although those algorithms have various forms, a general stereo matching procedure involves following four steps~\cite{stereo2002scharstein, stereo2003Brown}:
%\begin{itemize}
%    \item Feature extraction (FE);
%    \item Cost aggregation (CA);
%    \item Matching/disparity optimization (MO);
%    \item Disparity refinement (DR);
%\end{itemize}

%\subsection{DNN Algorithms in Stereo Vision}
%\label{subsec:cnn}
%
%Similar to the DNN architectures in other applications, a typical DNN in stereo vision is a stack of different computation layers~\cite{deconv_2011,Zeiler_2014_deconv}, such as \texttt{Conv}, \texttt{Maxpool}, \texttt{Relu}, \texttt{Deconv}, etc. Among them, \texttt{Conv} and \texttt{Deconv} are the most computationally intense operations. In \Fig{fig:cost_distribution}, we show the cost distribution of different steps and its major contributor. As \Fig{fig:cost_distribution} shows, \texttt{Conv} and \texttt{Deconv} consist of over 99\% of computations. They are the main focus in this paper, and we introduce them here. 
%
%\paragraph{\texttt{Conv} operation} A convolution operation can be mathematically expressed as below, assuming the stride is $1$: 
%\begin{multline}
%Out[x_o,y_o,c_o] = \sum_{c_i}^{C}  \sum_{k_{yi}}^{K} \sum_{k_{xi}}^{K} \ In[x_o+k_{xi},y_o+k_{yi},c_i] *\\ W[x_o+k_i,y_o+k_i,c_i, c_o]
%\end{multline}
%
%where $x_o$, $y_o$, $c_o$ are the dimensions in width, height and channel of the \textit{ofmap}, and $c_i$ is the dimension in channel of the \textit{ifmap}, $K$ is the dimensions of weights. The convolution operation for one value in a \textit{ofmap} is to compute the inner product between a weight with corresponding values in a \textit{ifmap}. Overall, \texttt{Conv} consists of 60\% of computations on average in \Fig{fig:cost_distribution}.
%
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.9\columnwidth]{Deconv.png}
%\caption{The unsampling operation in Deconvolution operation, assuming stride is $ 2 $.}
%\label{fig:deconv}
%\end{figure}
%
%\paragraph{\texttt{Deconv} operation} Deconvolution operation is similar to a common convolution with an additional step, upsampling \textit{ifmap}, before the convolution operation. \Fig{fig:deconv} shows a upsampling procedure. For a simple 2x2 \textit{ifmap} (as shown in the first block), each element's surroundings is filled with zeros to double the size of original \textit{ifmap}, as the blank squares shown in the second image block. After umsampling, the new upsampled \textit{ifmap} then goes through a regular convolution operation.
%
%As \Fig{fig:cost_distribution} shows, \texttt{Deconv} consists about 40\% of computation in Stereo Vision DNNs, except for \texttt{MC-CNN-arch}\cite{McCNN2015}. The main reason for deconvolution is to recover from the ``downsampling'' operations in previous \texttt{Conv} layers and to produce a result that is close to the original resolution. This operation has been used in many DNN in stereo vision\cite{NvStereo2018, GCNet2017, PSMNet2018, FlownetC2015} and also widely used in other neural networks as well, such as, generative adversial network (GAN)\cite{song2018GAN, Yazdanbakhsh2018GAN}.

%\subsection{Trade-off Exploration}
%\label{subsec:tradeoff}
%
%For a typical computer vision application, we need to address two aspects: responsiveness and accuracy. In this section, we explore the trade off between performance and computation cost across multiple stereo vision algorithms, both conventional algorithms and DNN algorithms. In the following paragraphs, we show the following insight:
%
%There is a trade-off between computation budget and accuracy. More accurate algorithms need high computation budgets.
%
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.7\columnwidth]{pareto.pdf}
%\caption{Trade-off between computation budget and accuracy. Note that, DNN methods are colored in green and conventional methods are colored in yellow. The darker the color, the higher the computation cost.}
%\label{fig:pareto}
%\end{figure}
%
%
%\paragraph{Trade-off on Budget and Accuracy} \Fig{fig:pareto} shows the computation cost and accuracy for a set of stereo vision algorithms~\cite{stereo2002scharstein, stereo2003Brown, SGBM2008HH, StereoClass2008, PSMNet2018, NvStereo2018, DispNet2015, GCNet2017,Elas2010Geiger}. We classify these algorithms into two classes, conventional algorithms (in yellow) and DNN algorithms (in green). As \Fig{fig:pareto} shows, the computation cost in DNN algorithms is typically 2-3 order of higher than conventional algorithms. The largest difference is almost $ 10^5 $ times higher. Even within the same class, the computation power could also be 1-2 orders of difference. This result strongly indicates that different algorithms are needed to be supported based on different user's computation budget and expected accuracy.
%
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.7\columnwidth]{testCategory.pdf}
%\caption{Computation accuracy of different DNN on different image categories.}
%\label{fig:performance}
%\end{figure}
%
%\paragraph{Use Scenario} In addition, we further characterize algorithms with equivalent accuracy in different use cases. \Fig{fig:performance} shows the accuracy variation of five different algorithms in different use cases.  We show two conventional algorithms, \texttt{SGBM}~\cite{SGBM2008HH} and \texttt{ELAS}~\cite{Elas2010Geiger}, and three DNN algorithms, \texttt{NV\_CNN}~\cite{NvStereo2018}, \texttt{PSMNet}~\cite{PSMNet2018} and \texttt{FlowNetC}~\cite{FlownetC2015}. We use the \textit{KITTI} and \textit{Monkaa} dataset and classify them into six different use cases.
%As \Fig{fig:performance} shows, two conventional algorithms all have low accuracy, but the accuracy of their algorithms under different use case changes dramatically. This also have been shown in the DNN algorithms with relatively less variations. For instance, \texttt{FlowNetC} has relatively low error rate on first five different use case, but have almost as double as the error rate of \texttt{NV\_DNN} on ``driving'' case.
%
%Results above clearly show that algorithms in both classes vary their accuracies on the different use cases. Therefore, it is needed to design a general framework for a broad range of stereo vision algorithms, instead of single one. 
%


==> ASV_ Accelerated Stereo Vision System/conc.tex <==
\section{Conclusion} 
\label{sec:conc}

%To achieve a high-precision and real-time stereo vision system, we have to improve on both ends: performance and energy. \proj effectively leverage the unique characteristics in Stereo vision by combining both classic and DNN algorithms. This paper points out the invariant in the stereo vision and unique transformation in stereo DNNs.

\proj simultaneously improves performance and energy-efficiency of ``depth from stereo'', while maintaining high accuracy. 
\proj combines algorithmic and computational optimizations that leverage characteristics unique to stereo vision. We demonstrate careful design choices that let these optimizations be integrated with existing DNN accelerators with minor hardware extensions. As intelligent machine perception increasingly relies on depth sensing, \proj provides a promising first step towards comprehensive system support.

==> ASV_ Accelerated Stereo Vision System/deconv.tex <==

% \begin{figure*}[t]
% \centering
% \includegraphics[width=\textwidth]{split_deconv.pdf}
% \caption{Translating deconvolution to a set of convolutions. Standard deconvolution first upsamples the \textit{ifmap} before convolving with the kernel. Note that this example assumes the upsampled \textit{ifmap} is not further padded before the convolution, i.e., a $7 \times 7$ \textit{ifmap} results in a $5 \times 5$ \textit{ofmap}. Our translation algorithm, however, holds generally regardless of padding.}
% \label{fig:split_deconv}
% \end{figure*}


\section{Deconvolution Optimizations}
\label{sec:deconv}

While the ISM algorithm removes DNN inference in non-key frames, DNNs remain critical for generating initial key frame correspondences. 
This section describes optimizations for stereo DNNs, in particular the dominant deconvolution layers. 
We propose novel software-only optimizations that mitigate the compute overheads in deconvolution (\Sect{sec:deconv:algo}), while capturing unique data reuse opportunities (\Sect{sec:deconv:reuse}).

We make our optimization framework publicly available at: \url{https://github.com/horizon-research/systolic-array-dataflow-optimizer}. It targets the systolic-array accelerator architecture, supports the deconvolution optimization described here, and applies tiling optimizations to minimize the inference latency and/or DRAM traffic.

\subsection{Deconvolution Transformation}
\label{sec:deconv:algo}

Deconvolution layers on average contribute to 38.2\% (50\% max) of the total MACs in stereo DNNs (\mbox{\Fig{fig:cost_distribution}}). 
Due to the inherent sparsity of deconvolution, a naive mapping to hardware results in over 75\% of redundant computations due to one or more zero operands. 
Deconvolution is also used in Generative Adversarial Networks (GANs), and recent studies have proposed specialized hardware specifically for deconvolution~\cite{song2018GAN, Yazdanbakhsh2018GAN}. 
In contrast to previous studies, we propose a \textit{purely algorithmic transformation} that eliminates inefficiencies due to sparsity. We show that an inherently sparse deconvolution layer can be translated to a series of dense convolutions, which then effectively map on to existing DNN accelerators. 
We next explain the inefficiencies in deconvolution, and then describe our algorithmic transformations.

\paragraph{Standard Deconvolution} The standard process (\Fig{fig:split_deconv}) deconvolves a 3x3 input feature map (\textit{ifmap}) with a 3x3 kernel. 
The \textit{ifmap} is first upsampled with zero padding, before being convolved with the 3x3 kernel to generate an output feature map (\textit{ofmap}). 
Note that the upsampling step essentially performs disparity refinement, which is fundamental to general stereo DNNs, rather than being specific to a particular network~(\Sect{sec:bcg:sv}). The zeros in the upsampled \textit{ifmap} leads to redundant computation and memory traffic.

%First, there are unnecessary MAC operations occurred in each \texttt{Conv} operation. In the case of $Out(1,1)$, there is only one effective MAC operation in the first 3x3 \texttt{Conv} operation. Second, some additional on-chip storage and memory traffic are incurred to store upsampled \textit{ifmap}.


%The key idea is that the sparse deconvolution operation can be effectively translated to a sequence of dense convolution operations. This translation is done in two steps that focus on mitigating the compute and memory wastes, respectively.

%We propose a simple algorithmic optimization that eliminates the redundant compute and data movement, without any hardware modifications. 

A key characteristic of deconvolution is that different elements in the \textit{ofmap} are calculated in different ``patterns.''
Consider the first $2\times 2$ outputs in the \textit{ofmap}: (1, 1), (1, 2), (2, 1), and (2, 2). 
Each of the four outputs is generated using a different set of elements from the kernel. 
For instance, (1, 1) requires only $e$ while (1, 2) requires $d$ and $f$. 
Critically, there are only four different patterns, which are repeated across the \textit{ofmap}. 
Pixels (4, 4) and (2, 2) are calculated using the same elements from the \textit{kernel}, as are (1, 1) and (5, 5), (1, 2) and (5, 4), as well as (2, 1) and (4, 5). 
Due to the various patterns needed to generate different output elements, deconvolution is clearly an ``irregular'' operation. 
Prior work~\cite{Yazdanbakhsh2018GAN} exploits the four unique computation patterns by augmenting a conventional DNN accelerator with custom hardware units.

\paragraph{Deconvolution Transformation} In contrast, we find that existing DNN accelerators already provide the necessary architectural substrate to efficiently execute the four different patterns. The key is to recognize that the four computation patterns are essentially four different convolutions, each convolving the original \textit{ifmap} with a distinct kernel that is part of the original kernel. For instance, (2, 2), (2, 4), (4, 2), and (4, 4) are generated by convolving $\begin{bsmallmatrix} a & c \\ g & i  \end{bsmallmatrix}$ with \textit{ifmap}. More generally, the deconvolution in~\Fig{fig:split_deconv} is calculated as:
\begin{equation*}
  \begin{bmatrix}
    a & b & c \\
    d & e & f \\
    g & h & i
  \end{bmatrix}
  \widehat{\circledast}
  ~I = \mathcal{G}(
  \begin{bmatrix}
    e
  \end{bmatrix}
  \circledast
  I, 
  \begin{bmatrix}
    d & f
  \end{bmatrix}
  \circledast
  I, 
  \begin{bmatrix}
    b \\
    h
  \end{bmatrix}
  \circledast
  I, 
  \begin{bmatrix}
    a & c \\
    g & i
  \end{bmatrix}
  \circledast
  I)
\end{equation*}

\noindent where $\widehat{\circledast}$ denotes the deconvolution operation, $\circledast$ denotes the standard convolution operation, $I$ is the \textit{ifmap}, and $\mathcal{G}$ is a gather operation to assemble the \textit{ofmap} from the results of the four convolutions. $\mathcal{G}$ is simply implemented as a set of load operations to the on-chip buffer. Essentially, our algorithm decomposes the original $3 \times 3$ kernel into four sub-kernels, each requiring a smaller dense convolution with the original \textit{ifmap}, which can be executed efficiently on a conventional DNN accelerator.

%We illustrate this in the lower half in \Fig{fig:split_deconv}. To compute the first 2x2 block of \textit{ofmap} (as numbered \circled{white}{1}), the effective MAC operations are shown at the top right of \Fig{fig:split_deconv}. As the equations show, each element has its own distinct convolution pattern, same as second 2x2 block (\circled{white}{2}). We make several observations:
%\begin{itemize}
%\item Cross-comparing \circled{white}{1} and \circled{white}{2}, there are four \texttt{Conv} patterns repeated in every 2x2 block.
%\item Each \texttt{Conv} pattern only use a certain subset of elements from original kernel. For instance, the first pattern (first element in 2x2 block) needs only element `e' (a sub-kernel notated as \circled{white}{i}) from the kernel.
%\item To compute one \texttt{Conv} pattern of the entire \textit{ofmap}, we only need a subset of original kernel (such as sub-kernel \circled{white}{i}) and compute \texttt{Conv} with the non-upsampled \textit{ifmap}.
%\end{itemize}

%Leveraging this observation, we first split the original kernel into four sub-kernels as shown in \Fig{fig:split_deconv}. Each sub-kernel then convolves with the original (un-upsampled) \textit{ifmap} to generate different elements that constitute the final \textit{ofmap}.

%and even 3D kernels~\mbox{\cite{NvStereo2018, GCNet2017, PSMNet2018}}
This transformation generalizes to kernel shapes other than \mbox{$3 \times 3$}. Formally, a 2D kernel $K$ with a dimension $K_H \times K_W$ will be decomposed into four sub-kernels ($S_0, S_1, S_2, S_3$):
% \vspace{-3pt}
\begin{align*}
    S_0^{(i,j)} & = 
                  K^{(2i,2j)}~~~~~~~~~~~~~
    i \in [0, \lceil K_H/2\rceil),
    j \in [0, \lceil K_W/2\rceil) \\
    S_1^{(i,j)} & = 
                  K^{(2i+1,2j)}~~~~~~~~~
    i \in [0, \lfloor K_H/2\rfloor),
    j \in [0, \lceil K_W/2\rceil) \\
    S_2^{(i,j)} & = 
                  K^{(2i,2j+1)}~~~~~~~~~
    i \in [0, \lceil K_H/2\rceil),
    j \in [0, \lfloor K_W/2\rfloor) \\
    S_3^{(i,j)} & = 
                  K^{(2i+1,2j+1)}~~~~~
    i \in [0, \lfloor K_H/2\rfloor),
    j \in [0, \lfloor K_W/2\rfloor) 
\end{align*}
%\begin{align*}
%    S^{(i,j)} = \left\{
%                \begin{array}{lll}
%                  K^{(2i,2j)} &
%    i \in [0, \lceil K_H/2\rceil),
%    j \in [0, \lceil K_W/2\rceil) \\
%                  K^{(2i+1,2j)} &
%    i \in [0, \lfloor K_H/2\rfloor),
%    j \in [0, \lceil K_W/2\rceil) \\
%                  K^{(2i,2j+1)} &
%    i \in [0, \lceil K_H/2\rceil),
%    j \in [0, \lfloor K_W/2\rfloor) \\
%                  K^{(2i+1,2j+1)} & 
%    i \in [0, \lfloor K_H/2\rfloor),
%    j \in [0, \lfloor K_W/2\rfloor) 
%                \end{array}
%              \right.
%\end{align*}

% \begin{align*}
%     \bigg\{~\overrightarrow{K_{sub}}~\bigg|~
%     \bigg(|K_{sub}^{(i)}| 
%         & \equiv~\lfloor |K^{(i)}|~/~2\rfloor~\land~ K^{(i,j)}_{sub}~\equiv~K^{(i,2j)}\bigg) \\
%     \lor~\bigg(|K_{sub}^{(i)}| 
%         & \equiv~ \lfloor (|K^{(i)}|+1)~/~2\rfloor ~\land~
%         K^{(i,j)}_{sub}~\equiv~K^{(i,2j+1)}\bigg) \\
%     & \forall~i~\in~|\overrightarrow{K}|~,~\forall~j~\in~
%     \lfloor|K^{(i)}|~/~2\rfloor 
%     \bigg\}
% \end{align*}

\noindent where $ S_{*}^{(i,j)} $ is the element $(i, j)$ in a particular sub-kernel, and $ K^{(*,*)} $ is an element in the original kernel $K$. For instance, $ S_0^{(i,j)} = K^{(2i,2j)} $ means that element $(i, j)$ in the first sub-kernel comes from element $(2i, 2j)$ in the original kernel. The boundary condition of each case denotes the dimension of the corresponding sub-kernel (notice the different floor and ceiling functions in each). Hence, decomposing a $3 \times 3$ kernel results in four sub-kernels of shapes $2 \times 2$, $1 \times 2$, $2 \times 1$, and $1 \times 1$, confirming the specific example above. The general formulation of the deconvolution transformation with an arbitrary N-dimensional kernel is described in \Apx{sec:appendix:decompose}.

%Similarly, a $N$ dimensional kernel in a deconvolution will be transformed into $ 2^N $ number of sub-kernels.
%For instance, in the first case, elements in this sub-kernel comes from the elements of the original kernel that are even-indexed at both dimensions, as we denote $ K^{(2i,2j)} $.
%To resolve this second issue, we introduce \texttt{Combine}. The idea is to combine four sub-kernels and batch them together in order to reuse the shared \texttt{ifmap}. By doing so, the \texttt{ifmap} stored in on-chip buffer can be fully utilized by all types of sub-kernels before flushing back to main memory. Potentially, we can deduct total memory traffic by 75\%, since most of memory traffic is due to \texttt{ifmap}.

% \paragraph{Co-compute Different Sub-kernels} Based on the dimensions of the kernel, we will yield different size of sub-kernels. In order to better utilize systolic array to reduce under-utilization, we pack small sub-kernel with large sub-kernel. Another benefit from this sub-kernel packing is that we can reduce the total data transfer from main memory to on-chip buffer. One side effect of this approach is that every MAC unit in the systolic array might need more than one register to hold the temporal result. To cope with this, our compiler can automatically synthesize the configuration that maximize the utilization of systolic array and minimizes the total data transfer.

\subsection{Exploiting Inter-Layer Activation Reuse}
\label{sec:deconv:reuse}

A beneficial trait of our transformation is that each sub-convolution reads the same \textit{ifmap}, which in modern DNNs does not fit in on-chip buffers and must spill to main memory. In contrast, our transformation can uniquely exploit \textit{inter-layer activation reuse} because each sub-convolution layer shares the same \textit{ifmap}. The challenge is to systematically maximize the reuse exploited across the entire network while minimizing the inference latency.

%A naive implementation of the translation would be to statically compile a deconvolution layer to a sequence of convolution layers. However, this implementation would increase the off-chip memory traffic. This is because each sub-convolution reads from the same \textit{ifmap}, 

We primarily consider \textit{loop tiling}, which is known to be critical to exploiting data reuse in DNNs~\cite{Mullapudi2016AutoHalide, yang2018dnn}. Prior work in DNN tiling predominately searches for the tiling strategy in a brute-force manner~\cite{Ma2017dnnFPGA, Hegde2018morph}. However, brute-force search does not scale to stereo DNNs for two reasons. First, our translation scheme significantly increases the number of layers, each of which must be individually searched. For instance in the example of \Fig{fig:split_deconv}, the number of layers quadruples; a 3D kernel could increase layers by $8\times$. Second, exploiting the inter-layer \textit{ifmap} reuse adds another scheduling dimension, further increasing the search space.

%In the previous section, we have shown how to convert \texttt{Deconv} operations into \texttt{Conv} and efficiently combine them. Based on our previous optimization scheme, we found that it is time-consuming and impractical to use exhaustive methods to iterate all configurations. Additionally, another dimension is introduced in the search space due to our \texttt{Deconv} optimization. Due to the vast and complexity of search space, naturally, we can use resource constraints in the existing hardware to trim the search space and accelerate the searching process. In this section, we present how to formulate the dataflow scheduling to be a constraint problem.

Instead of a search, we formulate the reuse optimization as a constrained optimization problem, minimizing layer latency while satisfying hardware resource constraints. Our optimization can be efficiently solved using a greedy algorithm.

%\begin{figure}[t]
%\centering
%\includegraphics[width=\columnwidth]{compute_pipe.pdf}
%\caption{Double-buffering overlaps the computation of the current round with the data accesses of the next round. The total latency is either compute-bound or memory-bound.}
%\label{fig:pipe}
%\end{figure}

\paragraph{Architectural Assumptions} We first describe the underlying architecture that the optimization formulation assumes. 
Overall, we make standard assumptions that generally hold across the vast majority of current DNN accelerators. \Sect{sec:sys:hw} describes the hardware architecture in detail.

We assume a systolic array accelerator. Each Processing Element (PE) performs one MAC operation per cycle~\cite{jouppi2017datacenter, samajdar2018scale}. Systolic arrays use a very efficient neighbor-to-neighbor communication mechanism, particularly well suited to convolution. Alternatively, our formulation could also be extended to support spatial arrays~\cite{Eyeriss2016}, which offer more flexible control at higher hardware cost.

%The buffer has its own address space and can be individually addressed. 
We assume that the accelerator has a unified on-chip buffer (scratchpad) for the \textit{ifmap}, kernels, and \textit{ofmap}. This buffer is generally too small to hold all the data for a whole layer. Therefore, the \textit{ofmap} is computed in multiple rounds. Only part of the \textit{ifmap} and the kernels are stored in the buffer each round. 
The optimal scheduling of partial \textit{ifmap} and kernels in the buffer for each round is critical to maximizing reuse.

The buffer is evenly split into working and filling sections for double-buffering. 
While the PE array is computing the current round using data in the working buffer, the data for the next round is pre-fetched to the filling buffer. The next round starts only when the filling buffer is full. This design choice guarantees that any data access by the PEs will hit in the buffer without stalling the PE array.

%Our dataflow optimization is based on our hardware design. In our design, a IP block like systolic array is used for computation and connected with a on-chip double-buffer. This double-buffer is aimed to overlap the execution of the computation and the data fetching from the main memory. The mechanism is shown in \Fig{fig:pipe}. The length of block represents the latency of different stages. For every time interval $t(i)$, the system spends $ L_{mem}(i+1) $ on fetching the necessary data (\textit{ifmap} and weights) from main memory. Meanwhile, the system overlaps the process of computing partial \textit{ofmap} (represented by $L_{comp}(i)$). The necessary data for this computation is pre-fetched during previous time interval, $t(i-1)$. Depending on the limits on different hardware resources, the bottleneck of this pipeline can be either by computation or memory accessing as shown in \Fig{fig:pipe}.

%A general scheme of DNN pipeline is to proceed layer-by-layer. For each layer, its dataflow can be classified into three main categories, input-stationary, weight-stationary, and output-stationary~\cite{Eyeriss2016, an2018scalesim}. Previous studies have shown three design considerations, \textit{loop blocking}, \textit{dataflow} and \textit{resource allocation}, affect the performance of DNNs~\cite{yang2018dnn}. In addition, it shows that it is \textit{loop blocking} within dataflow not \textit{dataflow} itself matters~\cite{yang2018dnn}. However, it is challenging to find the optimal computation ordering, considered the high dimension of computation space: \textit{ifmap}, \textit{ofmap} and weights. Therefore, current optimization routines usually rely on heuristics, which often leads to sub-optimal solution. In our framework, we propose a fast optimization routine that can achieve the optical dataflow solution using constraint optimization. In this paper, we mainly focus on output-stationary, however, the technique can be applied to other two categories as well.

\paragraph{Optimization Formulation} We follow a layer-wise execution model, in which a layer only starts after the previous layer finishes. Therefore, minimizing the total latency is equivalent to minimizing the latency of each individual layer. We describe how the latency of a deconvolution layer is formulated and optimized. Our formulation can be easily extended to support a convolution layer, which can be regarded as a special case of deconvolution without \texttt{ILAR}.

The optimization objective is to minimize the deconvolution layer's latency given hardware resource constraints. Note that since a deconvolution is translated to a set of convolutions, it is the cumulative latency of these sub-convolutions that is of interest. The optimization problem is formulated as follows:
\begin{align}
    \min\ &\ L(\Theta, \phi) \\
    s.t.\ &\ R(\Theta) \leq R^*
\end{align}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{tiling}
\caption{Tiling in a translated deconvolution with a $3 \times 3$ kernel split into four sub-kernels. With a tiling strategy $W=2, H=2, C_1=1, C_2=2, C_3=1, C_4=1$, only the shaded elements are loaded into the buffer. The \textit{ofmap} elements generated in this round (shaded) are also stored in the buffer.}
%\vspace{-15pt}
\label{fig:tiling}
\end{figure}

%We next formulate our constraint optimization. Our objective is to minimize the latency, $ L_{total} $, of the entire computation under a given hardware resource constraint. Based on our computation scheme, the latency of the entire DNN, $ L_{total} $, is the sum of the latency of each layer, $L^{(i)}$. 
%\begin{equation}
%L_{total} = \sum^{N}_{i=0} \{\min\ L^{(i)}(\Theta, \phi)\}
%\end{equation}
%Since the latency for each layer is independent under our execution model, our minimization operates on each layer individually. For simplicity, we only show the optimization of a single layer in the following formulations.

% \coloneqq \{{\theta^{(r)}}\}
\noindent where $\Theta$ denotes a particular hardware configuration, and $R(\cdot)$ is the configuration's hardware resources, which must not exceed the specified resource budget $R^*$. We consider three main types of hardware resources: 1) PE array size, 2) on-chip buffer size, and 3) off-chip memory bandwidth. 

Latency $L(\cdot)$ is affected by both the hardware configuration ($\Theta$) and the tiling schedule ($\phi$). The optimal tiling is determined by the following variables: 1) the dimension of the \textit{ifmap} tile to be loaded into the buffer ($W$ and $H$), and 2) the number of filters in each \textbf{sub-kernel $k$} to be loaded into the buffer ($C_k$). Critically, $C_k$ can be different for each sub-kernel. \Fig{fig:tiling} illustrates these optimization variables, with an example where part of the \textit{ifmap} is convolved with certain filters of the four sub-kernels to generate a partial \textit{ofmap}. 
The vector $\overrightarrow{C}$ denotes the collection of all $C_k$.

With double buffering, a layer $L$'s latency is the cumulative latency across all $N$ rounds. The latency of each round ($l^i$) is determined by the maximum value between the memory access time ($l^{i}_{m}$) and the compute time ($l^{i}_{c}$) of the round:
\begin{align}
L(\Theta, \phi) = \sum^{N}_{i=1} l^{i}(\Theta, \phi),~~~~~~l^{i}(\Theta, \phi) = \max(l^{i}_{c}, l^{i}_{m})
\end{align}

%\paragraph{Computation Ordering} 
%Based on our computation model, blocking of \textit{ofmap} has tightest data dependency and better explore locality~\cite{Mullapudi2016AutoHalide, yang2018dnn}. Therefore, in every computation process, we always compute the contiguous block of the \textit{ofmap} and further restrict this contiguous region to be a tile. This technique is often called as tiling. We notate the latency of computing a tile is $ l_{*} $ to distinguish from the latency of one layer, $ L_{*}$. In order to reduce the amount of data transfer between two tiles, we always compute adjacent tiles of \textit{ofmap}. The computation ordering within each tile would not affect the latency, assuming that the data can be always accessed on chip. However, the inter-tile ordering matters and affects the memory access latency, $ L_{mem} $.

%To reduce the total latency of computation, we reduce the enormous optimization space into two factors, the tile size of the \textit{ofmap} for each sub-kernel and the major computation ordering. For the computation ordering, there are two options: \textit{channel-major}, which computes \textit{ofmap} along the channel order first and \textit{row-major}, which is the row order first.

With double-buffering, $l^{i}_{c}$ is determined by two sets of parameters: 1) $W^{i}$, $H^{i}$, and $\overrightarrow{C^{i}}$, which decide the total compute demand, and 2) the PE array size, $A^*$, which decides the compute capability. $l^{i}_{c}$ is the cumulative latency of processing each individual sub-kernel:
\begin{align}
    %l^i_{c} & = \sum_{k=1}^{|\overrightarrow{C^i}|} \ceil{\frac{K^i_k(x) \times K^i_k(y) \times I \times C^i_k \times H^i \times W^i}{ A^*}}
    l^i_{c} & = \sum_{k=1}^{|\overrightarrow{C^i}|} \ceil{\frac{W^i_k \times H^i_k \times I \times C^i_k \times H^i \times W^i}{ A^*}}
\end{align}
\noindent where $|\overrightarrow{C^i}|$ denotes the total number of sub-kernels in round $i$, $W^i$ and $H^i$ are the dimensions of the \textit{ifmap} tile loaded into the buffer in round $i$, $W^i_k$ and $H^i_k$ are the dimensions of sub-kernel $k$ in round $i$\footnote{The sub-kernels' dimensions do not change across rounds. Given a $k$, $W^i_k$ and $H^i_k$ are constants for any $i$. For the consistency of the notations, we still use $W^i_k$ and $H^i_k$.}, $C^i_k$ denotes the number of filters in sub-kernel $k$ loaded into the buffer in round $i$, and $I$ is the number of input channels. The ceil operator indicates that the next sub-kernel can not start until the previous sub-kernel is finished even if the PE array is under-utilized. This is because only one sub-kernel can be calculated on the systolic array at a time as sub-kernels vary in their shapes.

The memory access time, $l^i_{m}$, is determined by the available memory bandwidth, $B^*$, and the amount of data that needs to be transferred to/from DRAM each round, which in turn depends on the reuse order: whether the \textit{ifmap} tile or the sub-kernels remain in the buffer across consecutive rounds. A binary variable $\beta$ denotes this reuse order, and $l^i_{m}$ becomes:
\begin{align}
    l^i_{m} & = \beta \times l^i_{m:W} + (1-\beta) \times l^i_{m:In},\ \beta \in \{0,1\}
\end{align}
where $ l^i_{m:In} $ is the memory access latency if the \textit{ifmap} remains in the buffer, and $l^i_{m:W}$ denotes the memory latency if the sub-kernels remain in the buffer. Specifically:
\begin{align}
    l^i_{m:W} & = \ (\Delta IF^i + \sum_{k = 1}^{|\overrightarrow{C^i}|} \Delta OF^i_{k}) \times\frac{1}{B^*} \\
    l^i_{m:In} & = \ \sum_{k = 1}^{|\overrightarrow{C^i}|} (\Delta W^i_{k} + \Delta OF^i_{k}) \times \frac{1}{B^*}
            %& \ where \ \  B \leq B^* \notag
\end{align}
\noindent where the terms with prefix $ \Delta $ denote the amount of data that needs to be loaded from DRAM. Depending on the reuse order, either the \textit{ifmap} elements ($\Delta IF^i$), or the sub-kernels ($\Delta W^i_k$) are loaded. The newly computed \textit{ofmap} elements ($\Delta OF^i_k$) are always stored back to DRAM. Note that $\Delta W^i_k$, $\Delta IF^i$, and $\Delta OF^i_k$ are all deterministic functions of $W^i_k$, $H^i_k$, $W^i$, $H^i$, and $|\overrightarrow{C^i}|$. We omit them here for brevity, and describe their exact expressions in~\Apx{sec:appendix:exp}.

The on-chip buffer capacity ($Buf^*$) imposes the constraint:
% stores all three categories of data, \textit{ifmap}, \textit{ofmap}, and weights. The total utilization of on-chip buffer is constrained by the current buffer capacity, which is expressed as below:
\begin{equation}
   \Delta IF^i + \sum_{k = 0}^{|\overrightarrow{C^i}|} (\Delta OF^i_k + \Delta W^i_k) \leq Buf^*
\end{equation}

Finally, $C^i_k$ and $N$ must satisfy:
\begin{align}
\forall k \in \{1, 2, ..., |\overrightarrow{C}|\}, \mathbb{C} = \sum^{N}_{i=1} C^i_k
\end{align}
\noindent where $\mathbb{C}$ denotes the number of output channels of a layer, which is a constant invariant to $k$ and $i$.

Overall, this formulation minimizes the latency $L$ with respect to $W^i$, $H^i$, and $C^i_k$ ($i \in \{1,2,...,N\}$, $k \in \{1, 2, ..., |\overrightarrow{C}|\}$), under the hardware resource constraints $A^*$, $B^*$, and $Buf^*$.

%To compute the latency of computing entire layer, we need to sum up the latency of each individual computation process. The number of computation process is subject to,
%
%\begin{equation}
%    N \leq |c_o^{(k)}| * |\overrightarrow{C_0}|
%\end{equation}

%where N is the number of batch needed to compute this layer, $ |C_o^{(k)}| $ is the number of kernel for a given sub-kernel and $ |\overrightarrow{C_0}| $ is the number of sub-kernel for a given layer.

%The overall optimization is summarized here:
%\begin{align*}
%    \min . & \sum_{i = 0}^{N} \{\max(L^{(i)}_{comp}, L^{(i)}_{mem})\} \\
%     with & \\
%          & \ L^{(i)}_{comp} = L^{(i)}(h_o, w_o, \overrightarrow{C_o}) \\
%          & \  L^{(i)}_{mem} = \phi * L^{(i)}_{W} + (1-\phi)*L^{(i)}_{In},\ \phi \in \{0,1\} \\
%    s.t.\ & \\
%          & \Delta ifmap +
%          \sum_{k = 0}^{|\overrightarrow{C_o}|} (\Delta ofmap^{(k)} + \Delta W^{(k)}) \leq Buf^*
%\end{align*}


%\subsection{Optimization on Block Matching}
%\label{subsec:bm_opti}

%\begin{figure}[t]
%\centering
%\includegraphics[width=0.6\columnwidth]{BM.pdf}
%\caption{Illustration of BM algorithm.}
%\label{fig:BM}
%\end{figure}

%In addition to mapping \texttt{Deconv} to systolic array, we also accelerate the key operation, block matching (BM), in conventional algorithms. BM is the most frequently used operation in conventional stereo vision algorithms~\cite{stereo2002scharstein, stereo2003Brown}, such as optical flow, stereo matching. 

%\paragraph{Block Matching} The main procedure in BM is to find the most similar block for a given image block in another image (see \Fig{fig:BM}). Given the image block with size of $ (h',w') $ in the left image at the coordinates $ (x,y) $, we want to find the most similar block with the same size in the right image. First, we define a searching window with $d \times d$ dimension at the coordinates $ (x,y) $ in the right image. Next, we scan through the $d \times d$ searching region to find the best similar block. The metric for best matching can be summed absolute difference (SAD) or weighted SAD of two matched blocks. The result with smallest SAD is the best match. Note that, in some algorithms, the searching region is defined only in one dimension. 
%
%The process is quite similar to \texttt{Conv} with some  differences:
%\begin{itemize}
%\item Instead of computing the element-size product in \texttt{Conv}, BM compute SAD. The convolution is only operated on a portion of \texttt{ifmap} instead of the entire one.
%\item BM has additional reduction to select the minimum SAD for every block. 
%\end{itemize}
%
%Due to those differences, we feature our new systolic array the capability of computing SAD, with a reduction unit on chip (\Sect{subsec:reduction_unit}).

% \begin{algorithm2e}
% \SetAlgoLined
% \KwIn{Layer $L$; Weights $W$; Buffer $Buf$.}
% \KwResult{Best c.latency $\in$  Config .}
% $W_{sub} = SplitDeconv(w_i) $\\
% $Config = PossiblePartition(Buf, L) $ \\
% \For{$c$ in $Config$} {
%     $ sol = 0 $ \\
%     $ W_s = W_{sub}.copy $ \\
%     \While {$W_s.notEmpty$} {
%         $r = \{\} $\\
%         \For{$w$ in $ W_s $}{
%             \tcp{Check if exceed constraint}
%             \If{SatConstraints($r$, $c$)}{
%                 break; \\
%             }
%             $ r.w = PackSubKernels(W_s) $ \\
%         }
%         \tcp{Use DP to reduce repeated compute}
%         $ sol$ += $ComputeLatency(r.w, c) $ \\
%         $ Rounds.append(r.w) $ \\
%     }
%     $c.latency = sol$\\
% }
% \caption{Deconv. Data-Reuse Optimization}
% \label{alg:opti}
% \end{algorithm2e}

\paragraph{Efficient Solver} The above constrained-optimization problem has non-convex objective and constraints, and thus has no closed-form solutions. To derive a solution efficiently, we convert this problem to a Knapsack-like structure, where each filter in each sub-kernel is an \textit{item}, the size of each filter is the \textit{weight}, and the number of MAC operations associated with each filter is the \textit{value}.

To solve the Knapsack problem, we use a simple greedy heuristic that prioritizes filters from large sub-kernels with standard dynamic programming. In contrast to the classic 0/1 Knapsack problem, our problem formulation requires us to consume all the items, since all the filters in each sub-kernel are required to finish a convolution. We therefore iteratively apply the greedy solver until all the items are used. The solver is executed offline, and finishes within one second on an Intel Core i5-7500 CPU.

%Based on the hardware constraints, we first generate a set of possible buffer partitioning options for each layer. For each option, the goal is to find the optimal packing strategy for sub-kernels under given hardware constraints. This problem can be formulated as classic Knapsack Problem. In this problem setting, . To solve this problem efficiently, we use a heuristic to always prioritize large sub-kernels and apply dynamic programming to avoid some redundant computations. 



% \Alg{alg:opti} shows the pseudo code of optimizing a single layer. In \Alg{alg:opti}, the solver initially transfers the deconvolution kernel into sub-kernels. Based on sub-kernels and hardware constraints, it searches for all possible buffer partitions, $ Config $. For each configuration, $c \in Config$, the solver calculates the number of rounds and the type of sub-kernels are in each round. Next, the solver accumulates the latency of this round to the total latency of this configuration. After calculating all the configurations, the solver return the best configuration from results. 

==> ASV_ Accelerated Stereo Vision System/disc.tex <==
\section{Discussion}
% What can I put in here?


==> ASV_ Accelerated Stereo Vision System/eval.tex <==
\section{Evaluation}
\label{sec:eval}

% \begin{figure}[t]
% \centering
% \vspace{-5pt}
% \includegraphics[width=\columnwidth]{ISM_result}
% \vspace{-15pt}
% \caption{Error rate comparison between the ISM algorithm in \proj and the DNN baselines.}
% \vspace{-13pt}
% \label{fig:ISM_result}
% \end{figure}

We first show that \proj adds negligible overhead to the baseline DNN accelerator (\Sect{sec:eval:oh}) and introduces negligible accuracy loss (\Sect{sec:eval:ac}). We then show the performance and energy improvements of \proj (\Sect{sec:eval:df}), which are robust against the underlying hardware configuration (\Sect{sec:eval:sensitivity}). \proj also out-performs Eyeriss and GPUs (\Sect{sec:eval:eyeriss}). Finally, we demonstrate the general applicability of our deconvolution optimizations by showing that they even improve runtime of GANs without hardware modifications (\Sect{sec:eval:gannx}).

\subsection{Hardware Overhead}
\label{sec:eval:oh}

Owing to the software transformations, \proj only minimally augments existing DNN accelerators. Relative to the baseline accelerator, \proj extends each PE to support accumulating absolute difference. This adds 6.3\% area (\SI{15.3}{\micro\metre\squared}) and 2.3\% power (\SI{0.02}{\milli\watt}) overhead \textit{per PE}. \proj also extends the scalar unit to support new point-wise operations, with an area and power overhead of \SI{2}{\mm\squared} and \SI{2.2}{\milli\watt}, respectively. The overall area and power overhead introduced by \proj are both below 0.5\%.

%PE area overhead: 0.14*0.063=0.00882 mm^2.
%scalar unit area overhead: 0.002 mm^2.

%\proj extends the controller (micro-code store) with \fixme{some entires}, and augments the scalar unit with logics to handle OF and BM-specific operations. Post layout synthesis results show a \fixme{XX}\% area overhead. The total area of \proj is about \fixme{XX}, commensurate with recent mobile-class CNN accelerators.

\subsection{Accuracy Results}
\label{sec:eval:ac}

\proj matches or even outperforms DNN accuracy.~\Fig{fig:ISM_result} shows the accuracy of applying the ISM algorithm to stereo matching DNNs. We use \textit{Propagation Window} (PW) to denote how far in time the correspondence invariant is propagated, which in turn decides how often key frames are selected. With PW-2, every other frame is selected as a key frame, and for PW-4, every fourth frame is a key frame. Note that the KITTI dataset contains at most two consecutive frames, and thus we evaluate only PW-2.

On both datasets, PW-2 retains the same accuracy as the stereo DNNs. On SceneFlow, PW-4 results in only 0.02\% accuracy loss. In some cases, ISM combined with the DNNs can outperform the DNNs alone. For instance, applying the ISM algorithm with \textsc{FlowNetC} reduces error by 0.11\% at PW-4. Overall, our experiments shows that by leveraging the correspondence invariant over time, ISM is able to preserve the DNN-like accuracy with cheap, classic stereo matching algorithms. We will now show that \proj achieves high accuracy while greatly improving the performance and energy-efficiency of stereo vision.

\subsection{Speedup and Energy Reduction}
\label{sec:eval:df}

\begin{figure}[t]
\centering
%\vspace{-5pt}
\includegraphics[width=\columnwidth]{asv_speedup_energy}
%\vspace{-15pt}
\caption{Speedup and energy reduction of the three \proj variants over the baseline.}
%\vspace{-13pt}
\label{fig:asv_result}
\end{figure}

\proj significantly improves performance and energy consumption of stereo vision. To understand the contributions of the ISM algorithm and the deconvolution optimizations,~\Fig{fig:asv_result} shows the speedup and energy reduction of the three ASV variants (\Sect{sec:exp:plan}) over the baseline, when applied to different stereo DNNs. We choose PW-4 for the ISM algorithm. On average, combining ISM and deconvolution optimizations (DCO) \proj achieves 4.9$\times$ speedup and 85\% energy reduction. Specifically, ISM achieves, on average, 3.3$\times$ speedup and 75\% energy reduction, while DCO achieves 57\% performance improvement and 38\% energy reduction. ISM contributes more than DCO because ISM avoids DNNs in non-key frames altogether by using the much cheaper BM and OF algorithms (\Sect{sec:algo:design}).

Next, we dissect different optimization components within DCO to further understand the effect of each optimization.

\begin{figure}[t]
\centering
\subfloat[Speedup and energy reduction on deconvolution layers only.]{
	\label{fig:dnns_deconv}
	\includegraphics[width=\columnwidth]{dnn_deconv_speedup_energy} }
%\vspace{-10pt}
\\
\subfloat[Speedup and energy reduction on the entire network.]{
	\label{fig:dnns_overall}
	\includegraphics[width=\columnwidth]{dnn_overall_speedup_energy} } 
%\vspace{-5pt}
\caption{The speedup and energy reduction of various deconvolution optimizations. Higher is better.}
%\vspace{-15pt}
\label{fig:dnns_result}
\end{figure}

\paragraph{Deconvolution Optimizations} Deconvolution optimizations consist of two components: the deconvolution to convolution transformation (\texttt{DCT} - \Sect{sec:deconv:algo}) and the data-reuse optimization (\Sect{sec:deconv:reuse}). In particular, our data-reuse formulation unifies the exploitation of two kinds of reuse: the conventional data reuse in convolution layers and the inter-layer activation reuse in deconvolutions that is uniquely exposed by \texttt{DCT}. To clearly tease apart our contributions, we show the results of both the conventional reuse optimization (\texttt{ConvR}), which is obtained by applying our reuse optimizer (\Sect{sec:deconv:reuse}) \textit{without} exploiting inter-layer activation reuse, and the additional effect of exploiting inter-layer activation reuse (\texttt{ILAR}).

\Fig{fig:dnns_result} shows the speedup and energy reduction of \texttt{DCT}, \texttt{ConvR}, and \texttt{ILAR}.~\Fig{fig:dnns_deconv} shows the improvements of deconvolution layers only, and~\Fig{fig:dnns_overall} shows the improvements of the entire network. The majority of speedup is from deconvolution transformation, which yields an average 3.9$\times$ speedup on deconvolution layers alone and 1.4$\times$ speedup on the entire network. On top of \texttt{DCT}, \texttt{ConvR} and \texttt{ILAR} further increase speedup to 5.6$\times$ and 1.6$\times$ on deconvolution layers alone and the entire networks, respectively.

%On average, all three techniques combined allow DCO to achieve a 5.6$\times$ speedup in deconvolution layers alone, and .

Across different stereo DNNs, we find that 3D DNNs (\textsc{GC-Net} and \textsc{PSMNet}) have a speedup of 7.7$\times$ on deconvolution layers, higher than the 3.9$\times$ speedup of 2D DNNs (\textsc{DispNet} and \textsc{FlowNetC}). The reason is twofold. First, 3D DNNs have the higher percentage of zero-padding than 2D DNNs (8$\times$ vs. 4$\times$), which are effectively eliminated by our deconvolution transformation. Second, after the deconvolution transformation the 3D DNNs have many small kernels (e.g., 1$\times$1$\times$1), which leads to low data-reuse. Thus, reuse optimizations become more critical to these networks. In contrast, most 2D stereo DNNs inherently have better data reuse with larger kernels (e.g., 5$\times$5). We also observe that \texttt{ConvR} and \texttt{ILAR} have similar performance. This is because both optimize the data reuse to the extent that the layer processing becomes limited by the PE size.

%Therefore, there are more opportunities for compute reductions in 3D DNNs. Second, higher compute reduction can potentially lead to reduction in memory access, there is less chance that DNN computation is stalled by memory access.

While \texttt{ILAR} is similar in speedup compared to \texttt{ConvR}, \texttt{ILAR} is much more effective in reducing energy than \texttt{ConvR}. To demonstrate this,~\Fig{fig:dnns_result} overlays the energy reductions of different DCO variants on the right $y$-axis. DCO achieves 83\% energy reduction on deconvolution alone and 38\% on the entire network. Specifically, \texttt{DCT} reduces the deconvolution energy by 62\%; \texttt{ConvR} and \texttt{ILAR} further improve the energy reduction to 73\% and 83\%, respectively.

The energy saving of \texttt{DCT} comes from eliminating redundant movement of padded zeros in the upsampled \textit{ifmap}. \texttt{ILAR} achieves additional energy reduction over \texttt{ConvR} by exploiting inter-layer activation reuse, a unique reuse behavior in our transformed deconvolution layers. 3D DNNs benefit much more from \texttt{ILAR} than 2D DNNs, as is evident by examining the additional energy reductions of \texttt{ILAR} over \texttt{ConvR} across networks. This is because 3D stereo DNNs have low \textit{ifmap} data-reuse; \texttt{ILAR} uniquely exploits inter-layer \textit{ifmap} reuse, and thus reduces more memory traffics.

\subsection{Sensitivity Analysis}
\label{sec:eval:sensitivity}

\begin{figure}[t]
  %\vspace{-10pt}
  \centering
  \captionsetup[subfigure]{width=0.5\columnwidth}
  \subfloat[\small{Speedup.}]
  {
  \includegraphics[width=.5\columnwidth]{profile_sensitivity_speedup}
  \label{fig:sensitivity_speedup_2d}
  }
  \subfloat[\small{Energy reduction.}]
  {
  \includegraphics[width=.5\columnwidth]{profile_sensitivity_saving}
  \label{fig:sensitivity_energy_2d}
  }
  %\vspace{-5pt}
  \caption{Sensitivity analysis of DCO speedup and energy reduction with buffer size and PE array size on \textsc{FlowNetC}. Speedup is normalized to the corresponding configurations, not to a single, common baseline.}
  %\vspace{-10pt}
  \label{fig:sensitivity_2d}
\end{figure}

While the speedup and energy reduction studied so far are based on one representative baseline accelerator configuration (\Sect{sec:exp:setup}), we find that our deconvolution optimization generally achieves similar improvements on other hardware configurations with resource provisions. In particular, we focus on two key types of hardware resource: PE size and on-chip buffer size. For brevity we only report results on \textsc{FlowNetC}~\cite{FlownetC2015}, but the trends generally hold.
%In this analysis, we normalize each configuration result to its corresponding SA-base. 

\Fig{fig:sensitivity_speedup_2d} and \Fig{fig:sensitivity_energy_2d} show how DCO's average speedup and energy reduction of the entire network  vary with different PE size and buffer size combinations, respectively. Note that the results are normalized to their corresponding hardware configurations rather than to the baseline described in \Sect{sec:exp:setup}. For instance, on the hardware with an 8$\times$8 PE array and a 0.5~MB on-chip buffer, DCO achieves an 1.44$\times$ speedup.

DCO achieves speedups of 1.2$\times$ -- 1.5$\times$ and energy reductions of 25\% -- 35\% across different hardware capabilities, demonstrating broad applicability. 
In general, the performance improvement of DCO is more pronounced with small PE arrays, where the performance is compute-bound. As the PE size increases, the performance becomes memory bound, such that memory bandwidth limitations mask the benefit of data reuse. In addition, as the buffer size increases, the reuse opportunities inherently exposed by the buffer is higher, and thus data reuse optimizations become less critical, hence the lower energy savings.

%The speedup and energy reduction are higher when the PE array size is small. This shows that, as the PE array becomes smaller, DCO optimization becomes more important. The reason behind it is that, as the PE size increases, there are less opportunities for data reuse optimization, thus, less space for DCO to explore. This is shown in both \Fig{fig:sensitivity_speedup_2d} and \Fig{fig:sensitivity_energy_2d}.
%Meanwhile, as the buffer size increases, there are more data reuse opportunities for DCO to explore, hence higher speedup as shown in \Fig{fig:sensitivity_speedup_2d}. However, \Fig{fig:sensitivity_energy_2d} shows that energy reductions is less sensitive to buffer size.

\subsection{Eyeriss and GPU Comparisons}
\label{sec:eval:eyeriss}

\begin{figure}[t]
%\vspace{-10pt}
  \centering
  \captionsetup[subfigure]{width=0.5\columnwidth}
  \subfloat[\small{Speedup.}]
  {
  \includegraphics[width=.5\columnwidth]{speedup}
  \label{fig:overall_speedup}
  }
  \subfloat[\small{Norm. energy. Lower is better.}]
  {
  \includegraphics[width=.5\columnwidth]{energy_saving}
  %\vspace{-10pt}
  \label{fig:overall_energy}
  }
  %\vspace{-5pt}
  \caption{Comparison of speedup and energy reduction for \proj, Eyeriss, and GPU. The results are normalized to Eyeriss. We show three variants of \proj. We also apply the deconvolution transformation to Eyeriss to obtain a stronger baseline, hence the \texttt{DCT} bar of Eyeriss.}
  \label{fig:overall_result}
  %\vspace{-5pt}
\end{figure}

For completeness, we also compare \proj with Eyeriss~\cite{Eyeriss2016} and a mobile Pascal GPU~\cite{tx2dev}.~\Fig{fig:overall_result} shows the speedup and energy reductions of the three \proj variants, Eyeriss and GPU. Data is normalized to Eyeriss. To obtain a stronger Eyeriss baseline, we extended the Eyeriss simulator~\cite{eyerisssim, gao2017tetris} to support our deconvolution optimization. Our ILAR optimization does not apply because Eyeriss's spatial architecture requires a different reuse formulation from the one presented here, which targets a systolic array.

On average, when combing DCO and ISM, \proj achieves $8.2\times$ speedup against Eyeriss while consuming only $16\%$ of the energy. DCO and ISM contribute to $38\%$ and $74\%$ on energy saving, respectively. Critically, Eyeriss can also benefit from the deconvolution transformation (\texttt{DCT}), which achieves a $ 1.6\times $ speedup and 31\% energy saving compared to the baseline Eyeriss. Finally, \proj is 27$\times$ faster while consuming 15$\times$ lower energy than the GPU.

\subsection{GANNX Comparison}
\label{sec:eval:gannx}

\begin{figure}[t]
  %\vspace{-10pt}
  \centering
  \captionsetup[subfigure]{width=0.5\columnwidth}
  \subfloat[\small{Speedup.}]
  {
  \includegraphics[width=.48\columnwidth]{gannx_speedup}
  \label{fig:gannx_speedup}
  }
  \subfloat[\small{Energy reduction.}]
  {
  \includegraphics[width=.48\columnwidth]{gannx_energy_saving}
  \label{fig:gannx_energy}
  }
  %\vspace{-5pt}
  \caption{Speedups and energy reductions on GANs between \proj and GANNX. Results are normalized to Eyeriss.}
  \label{fig:gannx_result}
  %\vspace{-10pt}
\end{figure}

Our deconvolution optimizations are not limited to stereo DNNs, but also apply broadly to deconvolution. To demonstrate general applicability, we apply the deconvolution optimizations to Generative Adversarial Networks (GANs), a class of DNNs that also make heavy use of deconvolution layers~\cite{goodfellow2014generative}. We compare against GANNX~\cite{Yazdanbakhsh2018GAN}, a dedicated DNN accelerator for accelerating deconvolution in GANs. We configure both \proj and GANNX to have the same PE and buffer sizes. We normalize the \proj results to Eyeriss, consistent with what GANNX reports.

\Fig{fig:gannx_result} shows speedup and energy comparisons across the six GANs used by GANNX. On average, \proj achieves $5.0\times$ speedup and $4.2\times$ energy reduction, higher than the improvements from GANNX ($ 3.6\times $ speedup and $3.2\times$ energy reduction). The higher gains from \proj are mainly attributed to the inter-layer activation reuse, which is uniquely exposed by our deconvolution transformation and is unavailable in GANNX. Critically, our deconvolution optimizations are purely software optimizations without requiring the specialized hardware support of GANNX.



==> ASV_ Accelerated Stereo Vision System/exp.tex <==
\section{Evaluation Methodology}
\label{sec:exp}

This section introduces the basic hardware and software setup~(\Sect{sec:exp:setup}), and outlines the evaluation plan~(\Sect{sec:exp:plan}).

\subsection{Basic Setup}
\label{sec:exp:setup}

\paragraph{Hardware Implementation} We develop validated RTL implementations for the \proj hardware. The hardware is based on a systolic array architecture, consisting of $24\times24$ PEs clocked at 1~GHz. Each PE is capable of performing both the MAC and absolute difference operations. The hardware also has a scalar unit clocked at 250~MHz, which consists of 8 parallel lanes, each capable of performing the ReLU activation function as well as the point-wise matrix update and compute flow operations required by OF. The on-chip buffer (SRAM) is 1.5~MB in size and is banked at a 128~KB granularity. While we primarily evaluate \proj using this configuration, we will later show sensitivity of \proj performance to different hardware resource configurations.

%Each SRAM read consumes 7.55 pJ and each write consumes 8.64 pJ. The SRAM leakage per bank is about 1~mW.

The RTL is implemented using Synposys synthesis and Cadence layout tools in TSMC 16nm FinFET technology, with SRAMs generated by an ARM compiler. Power is simulated using Synopsys PrimeTimePX, with full annotated switching activity. The off-chip DRAM is modeled after four Micron 16 Gb LPDDR3-1600 channels~\cite{micronlpddr3}. Overall, the accelerator layout has a total area of \SI{3.0}{\mm\squared}, and produces a raw throughput of 1.152 Tera operations per second.

\paragraph{Stereo DNNs} The ISM algorithm can use an arbitrary stereo DNN. We evaluate four state-of-the-art DNNs:  \textsc{FlowNetC}~\cite{FlownetC2015}, \textsc{DispNet}~\cite{DispNet2015}, \textsc{GC-Net}~\cite{NvStereo2018}, and  \textsc{PSMNet}~\cite{PSMNet2018}, with varying accuracy--performance trade-offs (\Fig{fig:trade-off}). %, and cover a wide range of input scenes (see \Fig{fig:usecases}).

\paragraph{Dataset} We evaluate \proj on two widely-used datasets: SceneFlow~\cite{DispNet2015} and KITTI~\cite{menze2015kitti}. SceneFlow contains 26 pairs of synthetic stereo videos to mimic various scenarios with different depth ranges. KITTI contains 200 pairs of stereo frames captured from real street views that cover varying driving scenarios and conditions. 

We use the standard ``three-pixel-error'' accuracy metric~\cite{menze2015kitti, kitti_benchmark}, which considers a pixel's depth to be correct if its disparity error is less than 3 pixels compared to ground truth. We then report the percentage of correct pixels, following the convention in the vision and robotics literature~\cite{PSMNet2018, NvStereo2018, DispNet2015, GCNet2017}.

%The execution speed is quantified by the frames-per-second, representing how fast the system generates depth estimations. The energy estimation includes the accelerator and the memory energy consumption.

%In addition, we also analyze the impacts of different hardware configurations on our design. In order to test the robustness of our design, we conducts the sensitivity analysis on the size of systolic array, the size of on-chip buffer and the memory bandwidth.


\begin{figure}[t]
\centering
%\vspace{-5pt}
\includegraphics[width=\columnwidth]{ISM_result}
%\vspace{-15pt}
\caption{Error rate comparison between the ISM algorithm in \proj and the DNN baselines.}
%\vspace{-13pt}
\label{fig:ISM_result}
\end{figure}

\subsection{Evaluation Plan}
\label{sec:exp:plan}

Our goal is to demonstrate the effectiveness of \proj over generic CNN accelerators that are not optimized for stereo vision workloads. We separate the efficiency gains of the new ISM algorithm from that of the deconvolution optimizations.

\paragraph{Baselines} Our baseline is a generic systolic array CNN accelerator, which executes stereo DNNs without any \proj optimizations. 
Today's CNN accelerators mostly statically partition the on-chip buffer across \textit{ifmap}, weights, and \textit{ofmap}. To obtain a strong baseline, we determine the partitioning strategy by exhaustively searching all the partitions offline and use the one that achieves the lowest latency for the entire DNN. Note that the same partition is used for all the layers whereas our data reuse optimization generates different partitions for different layers.
%We first study a typical configuration with a $16 \times 16$ PE array and a 1~MB global buffer. We then study the sensitivity of \proj under different PE array sizes and buffer sizes. 

We also compare against Eyeriss~\cite{Eyeriss2016}, a DNN accelerator based on a more flexible spatial architecture. Eyeriss performance and energy are obtained using the public simulator~\cite{gao2017tetris, eyerisssim}. For a fair comparison, we configure Eyeriss to have the same PE counts, on-chip memory capacity, and memory bandwidth as \proj. Finally, to establish a baseline, we also show the results of the Pascal mobile GPU found in the 16~nm Nvidia Parker SoC hosted on the Jetson TX2 development board~\cite{tx2dev}. We use the built-in power sensing circuity to obtain the energy consumption.
% and 59.7 GB/s memory bandwidth
%TX2 also exposes several SoC and board level power rails to a Texas Instruments INA 3221 voltage monitor IC, from which we retrieve power consumption through the I2C interface.

\paragraph{\proj Variants} We present an ablation study on \proj to separate the gains from different optimizations:

\begin{itemize}[topsep=0pt]
% \setlength\itemsep{-4pt}
  \item \mode{ISM}: ISM algorithm without deconv. optimizations.
  \item \mode{DCO}: Deconv. optimizations without ISM algorithm.
  \item \mode{ISM+DCO}: Both ISM and deconv. optimizations.
\end{itemize}


==> ASV_ Accelerated Stereo Vision System/intro.tex <==
\section{Introduction}
\label{sec:intro}

The demand for intelligent applications running on a diverse range of mobile and embedded platforms, such as micro-robots, augmented reality headsets, and smart-city sensor nodes, shows no sign of slowing down. 
A key primitive in these applications is estimating \textit{depth} information from the environment, which in turn serves as the building block for extracting higher-level semantics. 
For instance, depth information enables a mobile robot to detect and manipulate objects that are in close proximity.
%Similarly, a 3D mapping drone requires depth information to construct a model of the environment.

Among numerous depth sensing techniques, we focus on \textit{stereo} camera systems, which estimate depth from a pair of horizontally displaced cameras that capture two different views of the scene, mimicking the human binocular vision. 
%By projecting the same physical point to two corresponding pixels on two images, stereo vision algorithms calculate the horizontal offset between the two pixels (a.k.a. the \textit{disparity}), from which depth is estimated using the classical triangulation method~\cite{??}.
Compared to other depth sensing techniques such as LiDAR and structured-light sensors~\cite{wang20123d, weitkamp2006lidar}, stereo vision systems are much cheaper, consume less power, and are physically more compact~\cite{camera_comparison}. 
In response to the rising significance of stereo vision, recent mobile vision platforms integrate specialized stereo vision accelerators, such as the Stereo Depth Block in the Movidius Enhanced Vision Accelerator Suite~\cite{myriadx} and the Stereo \& Optical Flow Engine (SOFE) in the Nvidia Xavier mobile Systems-on-a-chip (SoC)~\cite{xaviersoc}.

%Computer vision has recently gained its use and popularity, thanks to the booming technology of silicon. The progress in computer vision also enables many applications, such as autonomous vehicles~\cite{NvStereo2018}, indoor navigation, robotics~\cite{suleiman2018navion} and high-precision 3D reconstruction, etc. These applications are or soon will be the norm in people's day-to-day life.

%One key for these applications is the ability to obtain the ambient information and estimate the depth of their surroundings. As human, we gather depth information of ambient from our two naked eyes. Being inspired by this idea, many applications use a stereo camera, a dual parallel-positioned camera, to capture a scene and apply a mathematical technique, triangulation, to compute the depth of the scene~\cite{lucas1981stereo}. People often categorize these applications into stereo vision.

%As much as is disclosed publicly, however, these stereo vision accelerators target classic stereo vision algorithms that use hand-crafted features that generally lead to low ac-curacies~\cite{??}.

%~\cite{stereo2002scharstein, stereo2003Brown, SGBM2008HH, StereoClass2008, Cech-CVPR-2011}
%Both the GPU and the accelerator provide around 1.2 TOPS raw throughput. 
Stereo vision algorithms presented to date broadly define a frontier in the accuracy-efficiency design space.
\mbox{\Fig{fig:trade-off}} compares the frame rate and accuracy for four well-known classic stereo algorithms that use ``hand-crafted'' features, including GCSF~\mbox{\cite{Cech-CVPR-2011}}, SGBN~\mbox{\cite{SGBM2008HH}}, HH~\mbox{\cite{SGBM2008HH}}, and ELAS~\mbox{\cite{Elas2010Geiger}}, as well as four state-of-the-art DNNs solutions~\mbox{\cite{PSMNet2018, NvStereo2018, DispNet2015, GCNet2017}}. 
The DNN data is characterized on both a Pascal mobile GPU~\mbox{\cite{tx2dev}} (``-GPU'' suffix), as well as on a DNN accelerator~\mbox{\cite{samajdar2018scale}} (``-Acc'' suffix). 
In using low-dimensional ``hand-crafted'' features, classic algorithms lead to high error rates ($x$-axis), but are compute efficient, mostly operating at close to real-time (e.g., 30~FPS, $y$-axis).
In contrast, DNNs models achieve very low error rates, but require 2--5 orders of magnitude more arithmetic operations, resulting in much lower frame rates.


%but have high error rates ($x$-axis) compared to DNNs. 
%At the same time, classic algorithms are compute-efficient. 

%By explicitly modeling the physical world and the image formation process~\cite{stereo2002scharstein, stereo2003Brown}, classic algorithms mostly operate close to real-time (e.g., 30~FPS), but lead to high error rates. 
%DNNs require 2--5 orders of magnitude more arithmetic operations than that of classic algorithms, leading to significantly lower frame rate.
%For instance, \textsc{FlowNetC}~\cite{FlownetC2015} operates at a meagre 2.3 FPS on a mobile Pascal GPU, and a dedicated CNN accelerator improves the frame rate to only 9.1, still a long way from real-time.

%On the other hand, simply using accuracy to trade for performance is also not applicable. \Fig{fig:sensitvity_disp} shows the depth mis-calculation of objects from varying distances. The depth mis-calculation can be due to the accuracy loss introduced by stereo camera. In~\Fig{fig:sensitvity_disp}, the data are collected from a commercial stereo camera, bumblebee2 (v1394a)~\cite{bumblebee2} with focal length of 3.8 mm. \Fig{fig:sensitvity_disp} shows that a pixel deviation of 0.2 accruacy loss in pixel will lead to 1m to 1.5m difference in actual depth for a object at distance between 10m to 15m. This might lead to lethal consequences in real-world applications.

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.7\columnwidth]{runtime}
% \caption{\proj achieves real-time (30 FPS) frame rate while retaining DNN-like accuracy.}
% \label{fig:trade-off}
% \vspace{-10pt}
% \end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.7\columnwidth]{trade-off}
\caption{\proj demonstrates both real-time (30 FPS) frame rates and DNN-like accuracy for stereo vision.}
\label{fig:trade-off}
%\vspace{-10pt}
\end{figure}
 
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.7\columnwidth]{dnn_benchmark.pdf}
%\caption{Computation accuracy of different DNN on different image categories.}
%\label{fig:usecases}
%\end{figure}

%In addition, we further characterize algorithms with equivalent accuracy in different use cases. \Fig{fig:performance} shows the accuracy variation of five different algorithms in different use cases.  We show two conventional algorithms, \texttt{SGBM}~\cite{SGBM2008HH} and \texttt{ELAS}~\cite{Elas2010Geiger}, and three DNN algorithms, \texttt{NV\_CNN}~\cite{NvStereo2018}, \texttt{PSMNet}~\cite{PSMNet2018} and \texttt{FlowNetC}~\cite{FlownetC2015}. We use the \textit{KITTI} and \textit{Monkaa} dataset and classify them into six different use cases.
%As \Fig{fig:performance} shows, two conventional algorithms all have low accuracy, but the accuracy of their algorithms under different use case changes dramatically. This also have been shown in the DNN algorithms with relatively less variations. For instance, \texttt{FlowNetC} has relatively low error rate on first five different use case, but have almost as double as the error rate of \texttt{NV\_DNN} on ``driving'' case.

%%%Many studies have investigated on stereo vision and introduced new algorithms originally by combining hand-crafted features and disparity optimization methods~\cite{Elas2010Geiger, SGBM2008HH, StereoClass2008, stereo2002scharstein, stereo2003Brown}. With the extraordinary achievements of deep neural network (DNN) and machine learning, new DNN architectures have been proposed and gained unprecedented improvements on accuracy~\cite{McCNN2015, DispNet2015, GCNet2017, FlownetC2015, PSMNet2018}. 

%%%However, DNN algorithms also have longer latency and higher computation cost, which drains current mobile battery even faster. For many real-time applications, accuracy and timing are two primary concerns. Therefore, it is important to address both reliability and responsiveness for stereo vision.

%However, the flexibility to support different algorithms is critical to stereo vision in the real world. To highlight the importance of flexibility,~\Fig{fig:performance} compares the accuracies of five state-of-the-art stereo DNNs when applied to six different visual scenes. Although \textsc{FlowNetC} achieves the overall best accuracy, \textsc{DispNet} and \textsc{NVCNN} are needed to maximize accuracy in the MultiObjects and Driving scenarios, respectively, underlining the need of flexibility.
%For a typical object at distance between 10m to 15m, the slight difference in disparity will lead to 2m to 2.5m difference in depth calculation, which is intolerable for real-world applications.

%This paper argues that stereo vision systems do not need to trade accuracy with compute-efficiency. 
This paper presents \proj, an accelerated stereo vision system that operates in real-time while achieving DNN comparable accuracy. 
While today's vision accelerators are primarily built for monocular vision tasks, \proj exploits unique characteristics of stereo vision, and applies stereo-specific optimizations, both algorithmic and computational. 
Critically, we show that with careful algorithmic choices, these stereo-specific optimizations can largely be implemented on the same computer architecture as conventional DNN accelerators with a set of basic, yet principled, hardware extensions, which widens the applicability of this work.

%We systematically examine the redundancies throughout the system stack, and propose a set of optimizations that mitigate the inefficiencies. 

%In this paper, we present a framework, \textit{Stereo Engine}, that leverages the unique characteristics in stereo vision and supports a wide range of algorithms in this domain. Comparing to previous studies, we highlighted some key features in our framework and some challenges that we solved within following paragraphs.

At the core of \proj is a new low-latency, high-accuracy stereo vision algorithm. 
We exploit the temporal invariance introduced by stereo cameras: a single physical point projects to a unique pair of pixels on the left and right image planes; although the pixel locations move over time, their corresponding geometric relationship is fixed.
Our algorithm, ISM, uses compute-intensive DNNs to extract pixel correspondences from a small set of key frames. 
The correspondences are then propagated as initial estimates for subsequent non-key frames, where we make use of cheaper, classic algorithms. 
By combining learnt features from DNNs, and classic algorithms that explicitly model the physical world, ISM achieves high accuracy while reducing the compute cost.

%The correspondence invariant allows us to use the depth information obtained from the current frame to guide the depth estimation in subsequent frames, simultaneously simplifying computation while improving accuracy.


% We recognize that stereo vision algorithms fundamentally require matching corresponding pixels in the left and right images. Classic stereo algorithms rely on some sort of search-based heuristics such as the search window and matching criterion for pixel matching. In contrast, DNN algorithms implicitly learn the searching heuristics through the massive features, but come at the expense of compute cost. Our idea is to guide the search process of the classic algorithm using DNN information rather than relying exclusively on either. In other words, DNNs provide ``hints'' to improve the search heuristics of classic algorithms, achieving high efficiency and high accuracy at the same time.

%\textit{First, we propose a new algorithm that combines the methods in both conventional and DNN algorithms to improve responsiveness while maintaining high accuracy.} For human, we often perceive the information of surroundings in an incremental way. We first have a primitive sense of the entire scene. Next, We incrementally gain our knowledge based on the changes of environment. This inspires us reuse previous result and simplify the computation process. Although, previous studies have adopted this idea and used motion compensation to extrapolate the result~\cite{EVA2,zhu2018isca}. In our framework, the situation is different, and the key enabler is to leverage a unique step in stereo vision, triangulation, to obtain an accurate result similar to the result from DNN algorithms with much shorter latency.

While our ISM algorithm reduces the compute overhead, DNNs remain critical, as they generate the initial estimate of the correspondence information. 
We observe that stereo DNNs make heavy use of the \textit{deconvolution} operation\footnote{Deconvolution in deep learning is an incredibly unfortunate misnomer that should really be called ``transposed convolution.''} that exposes specific kernel sparsity, making conventional DNN accelerators inefficient. 
While prior work proposed specialized hardware to exploit deconvolution sparsity~\mbox{\cite{song2018GAN,Yazdanbakhsh2018GAN}}, we demonstrate that static software optimizations achieve better results without unnecessary hardware modifications.

Our approach is to transform an inherently sparse deconvolution layer into a sequence of dense convolutions, which can then be executed by canonical DNN accelerators. 
More importantly, this transformation uniquely exposes a new data reuse opportunity: \textit{inter-layer activation reuse} (ILAR), which does not exist in conventional DNNs.
While exhaustive search has been previously used to optimize data reuse patterns, it does not scale to optimizing deconvolution, because the transformation increases the layer count by up to 8$\times$, and ILAR adds another search dimension. 
Instead, we propose a constrained-optimization formulation, and demonstrate an efficient solver using dynamic programming.

We implement a software/hardware co-designed prototype of \proj. 
The hardware builds on top of a conventional systolic DNN accelerator~\cite{jouppi2017datacenter} implemented in 16nm technology. The \proj hardware minimally extends the baseline accelerator with less than 0.5\% area overhead. 
The software integrates the ISM algorithm and the deconvolution optimizations.

We evaluate \proj on a set of standard stereo vision benchmarks. Compared to the DNN baseline, \proj achieves 5$\times$ speedup and 85\% energy saving with 0.02\% accuracy loss. We also demonstrate the general applicability of software deconvolution, by applying it to Generative Adversarial Networks (GANs), which also make heavy use of deconvolutions. Under the same compute and memory resource constraints, we achieve 1.4 $\times$ speedup over a purpose-built deconvolution accelerator, due to the unique ILAR that we exploit.

%\textit{Second, we proposed a unified hardware that is based on systolic array and supports key operations in both conventional and DNN algorithms.} Although, many studies have already proposed hardware accelerators on DNN algorithms, by using varying techniques, such as, quantization and data compression\cite{EIE2016}, elimination of redundant computation\cite{SnaPEA2018}, increasing data locality by layer fusion\cite{FusedCNN2016} or manipulating data flow\cite{DaDianNao2014, Eyeriss2016}, etc. However, directly applying these accelerators on stereo vision, we observed two fundamental limitations, which we address in our design. First, most of accelerators are contextually agnostic and cannot leverage some unique information in DNN algorithms to avoid unnecessary computation. Second, in order to support operations in non-DNN algorithms, one additional piece of hardware is needed~\cite{song2018GAN,Yazdanbakhsh2018GAN}, which increases the chip area. In our design, we realize the common compute patterns in stereo vision algorithms and map them in a unified systolic-array-like hardware. By doing so, our hardware design guarantees its generality and performance meanwhile avoids unnecessary computation.

%\textit{Third, we proposed a unique optimization routine for DNN dataflow without any heuristics from previous studies.} In previous studies, different heuristics have been used to explore the locality and reduce the compute time, such as unrolling, tiling, loop re-ordering~\cite{Mullapudi2016AutoHalide, Mullapudi2015Polymage, yang2018dnn}. Others also explore different data-stationary strategies to reduce the latency~\cite{Eyeriss2016, an2018scalesim}. However, using heuristics often results in a sub-optimal configuration of DNN dataflow given a particular hardware substrate. In this paper, we reduce the dataflow optimization into a non-linear constraint optimization and solver the optimization using off-the-shelf solver~\cite{??}. Comparing to previous studies, Our framework avoid using heuristics, and it can find better dataflow procedure in less time and achieve better runtime performance.

To our best knowledge, this is the first paper that demonstrates a cost-effective stereo vision system. 
Using a software-hardware co-design approach, we show that carefully designed software optimizations achieve significant performance and energy improvements with simple, principled changes to existing DNN accelerators, which widens the applicability of our work. More specifically:

%simultaneously improves both the compute-efficiency and accuracy of state-of-the-art DNN approaches
\begin{itemize}[topsep=0pt]
% \setlength \itemsep{-3pt}
\item We propose the first stereo vision algorithm, ISM, that exploits \textit{temporal invariance} in stereo imaging to improve the performance with minimal accuracy loss;
\item We propose the first \textit{static} optimization framework for deconvolution, a key operation in stereo DNNs, which eliminates the sparsity-induced compute inefficiencies in deconvolution layers without hardware changes;
\item We are the first to identify \textit{inter-layer activation reuse} in deconvolution, \textit{a unique data reuse opportunity} exposed by our transformation framework, and which we exploit using an efficient constrained optimizer.
\item We co-design the hardware with the proposed software optimizations to achieve fast, low-power stereo vision \textit{with minimal changes to existing DNN accelerators}.
\end{itemize}

The remainder of the paper is organized as follows.~\Sect{sec:bcg} gives an overview of necessary background.
\Sect{sec:algo} introduces our invariant-based stereo matching algorithm.
\Sect{sec:deconv} describes the software optimizations for efficient implementation of the deconvolution operation.
\Sect{sec:sys} presents the design of \proj, including both software and hardware considerations.
\Sect{sec:exp} and \Sect{sec:eval} are experimental methodology and results, respectively.
\Sect{sec:related} positions \proj in the context of related work, and \Sect{sec:conc} concludes the paper.



==> ASV_ Accelerated Stereo Vision System/macros.tex <==
%!TEX root=paper.tex

\newcommand{\website}[1]{{\tt #1}}
\newcommand{\program}[1]{{\tt #1}}
\newcommand{\benchmark}[1]{{\it #1}}
\newcommand{\fixme}[1]{{\textcolor{red}{\textit{#1}}}}

\newcommand*\circled[2]{\tikz[baseline=(char.base)]{
            \node[shape=circle,fill=black,inner sep=1pt] (char) {\textcolor{#1}{{\footnotesize #2}}};}}

\ifx\figurename\undefined \def\figurename{Figure}\fi
\renewcommand{\figurename}{Fig.}
\renewcommand{\paragraph}[1]{\textbf{#1}~~}
\newcommand{\figline}{{\vspace*{.05in}\hline}}

\newcommand{\Alg}[1]{Alg.~\ref{#1}}
\newcommand{\Sect}[1]{Sec.~\ref{#1}}
\newcommand{\Fig}[1]{Fig.~\ref{#1}}
\newcommand{\Tbl}[1]{Tbl.~\ref{#1}}
\newcommand{\Equ}[1]{Equ.~\ref{#1}}
\newcommand{\Apx}[1]{Appendix~\ref{#1}}

\newcommand{\specialcell}[2][c]{\begin{tabular}[#1]{@{}l@{}}#2\end{tabular}}
\newcommand{\note}[1]{\textcolor{red}{#1}}

\newcommand{\greenweb}{{\fontfamily{cmtt}\selectfont GreenWeb}\xspace}
\newcommand{\autogreen}{\textsc{AutoGreen}\xspace}
\newcommand{\proj}{\textsc{ASV}\xspace}
\newcommand{\mode}[1]{\underline{\textsc{#1}}\xspace}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}

\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}

% checkmark and xmark in the pifont package
%\newcommand{\cmark}{\ding{51}}
%\newcommand{\xmark}{\ding{55}}


==> ASV_ Accelerated Stereo Vision System/overview.tex <==

\begin{figure*}
\centering
\begin{minipage}{.4\textwidth}
  \centering
  \includegraphics[width=\linewidth]{overview}
  \captionof{figure}{Overview of our framework.}
  \label{fig:overview}
\end{minipage}%
\begin{minipage}{.6\textwidth}
  \centering
  \includegraphics[width=\linewidth]{motion_algorithm}
  \captionof{figure}{Comparison of DNN pipeline with our integrated pipeline.}
  \label{fig:motion_algorithm}
\end{minipage}
\end{figure*}

\section{System Overview}

As we shown in \Sect{subsec:tradeoff}, it is necessary to design a stereo vision framework that supports a range of stereo vision algorithms. Meanwhile, to achieve the global optimal in the design space, we co-design algorithm and hardware to fully explore the unique characteristics of stereo vision. Here, we overview our design in three dimensions: algorithm, compiler and hardware, and explain how each component collaborate with others. 

\Fig{fig:overview} shows the stack of our design. At the top of our stack, a stereo vision runtime serves as an interface to varying stereo vision applications. To support different DNN algorithms, we design our stereo vision runtime that can embed any stereo vision applications with our integrated algorithms. At the bottom of our stack, we designed our stereo engine to support any computations in both classic and DNN algorithms in stereo vision pipelines. The key to bridge the runtime and the hardware is our compiler. Our compiler can automatically map any operation in algorithms onto the hardware. Meanwhile, our compiler optimizes the dataflow of stereo vision program and the hardware configuration to a global optimal under some constraints of hardware recourse. Next, we shortly highlight key features of each components in our framework, more details are in later sections.

\paragraph{Integrated Algorithm} As we have shown in \Sect{subsec:tradeoff}, on one hand, the state-of-the-art DNN algorithms are accurate but computationally expensive for most commodity devices, on the other hand, conventional algorithms are faster but poor in accuracy. In order to reduce the latency of DNN algorithms, we propose a runtime algorithm that couples DNN algorithms with the idea, triangulation, from conventional algorithms. By combining the merits of both, our runtime can achieve a substantial improvement on runtime performance and energy saving without substantial accuracy loss.

\paragraph{Hardware Support} To support varying operations in both conventional and DNN algorithms, we modify the classic design of systolic array. The modified systolic array can support all the key operations in both algorithms. We want a unified hardware instead of one hardware for each algorithm or operation. In addition, we design a memory controller to help with managing the dataflow on and off the chip. The overall design lets us avoid separate IP blocks per operation and some redundant computations, such as in \texttt{Deconv}. Previous studies have proposed special IP blocks to avoid the computational redundancy in \texttt{Deconv}~\cite{song2018GAN, Yazdanbakhsh2018GAN}. However, additional hardware for \texttt{Deconv} is hardly acceptable, especially on mobile platforms.

\paragraph{Compiler Optimization} 
In our design, the compiler has two key features. First, it can map the key operations in stereo vision algorithms to the modified systolic array. Second, our compiler conducts an unique dataflow optimization using constraint optimization. Doing this transformation, our compiler can use off-the-shelf solvers to configure the optimal dataflow for a particular hardware.




==> ASV_ Accelerated Stereo Vision System/plan.tex <==
\section{Outline}
\begin{itemize}
\item Background 
\begin{enumerate}
\item Stereo vision: introduce two parts: the general procedure of stereo matching, and triangulation to compute depth map from disparity map.
\item CNN: introduce general CNN convolution and address 3D CNN in some stereo matching DNN. Last, introduce deconvolution layer.
\end{enumerate}

\item Motivation: show the trade-off between computation and performance. Different use scenarios need to use different DNN based on DNNs latency and accuracy.

\item{Optimization}
\begin{enumerate}
\item Dataflow optimization: by changing the dataflow, the total latency of entire computation can be dramatically reduced. We propose two type of dataflow optimization comparing to previous studies. 
\begin{itemize}
\item First, we based on a typical CNN, we propose a algorithm pipeline to accelerate the entire CNN computation. 
\item Second, based on the unique character of deconvolution, we propose a new way to compute with a HW support.
\end{itemize}

\item Algorithm-level optimization: Further exploring the trade-offs between accuracy and performance, we leverage two unique characteristics on stereo vision.
\begin{itemize}
\item Use triangulation to leverage the result from the previous frames and reduce the computation cost of DNN.
\item Most of stereo matching DNN pipeline, in their deconvolution stage, will compute a small-scale result and fine-tune it at later stages. We take advantage of this characteristics and use simple extrapolation to compute fine-grained result.
\end{itemize}

\end{enumerate}  % optimization



\item Hardware support 
\begin{enumerate}
\item Modification on systolic array: to have 4 registers per MAC unit and a signal controller to signal which register should store the current computed value.
\item Buffer controller: control the partition of buffer lane and load/store of each buffer lane.
\end{enumerate}

\end{itemize}

















==> ASV_ Accelerated Stereo Vision System/related.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Stereo Vision Accelerators} Recently, commercial mobile vision systems~\cite{Zhu2018mlsoc} have started integrating dedicated stereo accelerators, such as the Stereo Depth Block in the Movidius Enhanced Vision Accelerator Suite~\cite{myriadx}, and the Stereo \& Optical Flow Engine (SOFE) in the Nvidia Xavier mobile SoC~\cite{xaviersoc}. From publicly available details, these are fixed-functioned accelerators targeting classic stereo algorithms, similar to previous stereo vision accelerators~\cite{mazumdar2017exploring, wang2015real_time_stereo_system,  gudis2013stereoembedded, ttofis2014high, yang2014hardware}. In contrast, \proj combines the efficiency of classic stereo algorithms with the accuracy of stereo DNNs.

%With the rising popularity of high-precision stereo vision applications, many studies have proposed new vision accelerators or embedded stereo vision system on FPGA for classic algorithms. Unlike prior work, our work integrates both classic and DNN-based algorithms and supports general stereo vision instead of specific algorithms.  We envision that more stereo vision-specific accelerators will appear to support algorithms on both ends.

%However, prior motion-based algorithms are designed for monocular vision tasks that operate on single images. Stereo vision exposes unique challenges to which prior motion-based algorithms do not apply. Specifically, 
\paragraph{Motion-based Algorithms} Our ISM algorithm shares a similar key observation as some recent motion-based vision algorithms such as EVA$^2$~\cite{buckler2018eva2} and Euphrates~\cite{zhu2018euphrates}, in that correlation across frames in a video stream
can be used to simplify continuous vision tasks. Euphrates~\cite{zhu2018euphrates} focuses on computing regions-of-interest (ROIs) in object detection and tracking tasks. In contrast, stereo vision is concerned with the depth of the whole frame rather than discrete ROIs. 
EVA$^2$~\cite{buckler2018eva2} is not limited to ROIs. However, it relies on estimating the motion of an intermediate activation's receptive field. In the stereo task, the receptive field of an intermediate activation necessarily spans both the left and right images. Thus, the motion of the receptive field would be difficult, if not impossible, to calculate.

%Our algorithm leverages the unique characteristics of stereo vision to propagate the matching pair information through the motion of both left and right images, avoiding the need for motion estimation in receptive fields or ROIs that is unobtainable in stereo vision networks.

Fundamentally, motion-based relaxations fall within the realm of incremental computing, a general technique used in program analysis
and optimization~\cite{michie1968memo, pugh1989incremental} and applies beyond the temporal and/or vision domain. 
Diffy~\cite{mahmoud2018diffy} exploits the spatial similarity across pixels in the same frame to improve DNN efficiency. Riera et al.~\cite{riera2018computation} exploit repeated \textit{ifmap} elements in speech recognition.

\paragraph{Deconvolution Sparsity} Many prior studies optimize hardware to exploit sparsity in DNNs~\cite{shiftnet2018, wen2016learning_Sparsity, He2017channel_pruning, kung2018packing, Parashar2017scnn, lee2019sparse, whatmough2018sparse, Cnvlutin2016, EIE2016}. 
Stereo vision DNNs make use of deconvolution layers, which expose structured sparsity patterns. 
Recent work has prosed specialized hardware specifically for exploiting sparsity in deconvolution layers~\cite{Yazdanbakhsh2018GAN, song2018GAN}. Our observation, however, is that mitigating sparsity-induced efficiencies in deconvolution does not necessarily require hardware support. We propose novel software optimizations to eliminate the compute inefficiencies without hardware changes.

%Some prior work show that weight pruning can effectively remove large percentage of weight without significant accuracy loss. However, weight pruning generally needs re-training while pruning the network for each DNN\cite{wen2016learning_Sparsity, He2017channel_pruning, kung2018packing}. Other work have proposed new microarchitectures can adapt model compression~\cite{EIE2016} or skip ineffective zero-products in convolution~\cite{Cnvlutin2016, Parashar2017scnn}. However, their performance improvements heavily depend on compression rates and data irregularity, which is orthogonal to our work. one important point is that all the work above have not yet explored the unique characteristics in deconvolution, which has a regular compute pattern. Based on this characteristic, previous studies propose some special DNN accelerators to support deconvolution during training~\cite{song2018GAN} or inference~\cite{Yazdanbakhsh2018GAN}. However, these prior work need to modify the micro-architecture which imposes additional area overhead. 

%Different from others, we propose \proj, a pure software implementation to achieve a better performance with a tiny modification on hardware. This is important especially for mobile devices while area is crucial.

\paragraph{Data-Reuse Optimization} Exploiting data-reuse (through tiling) is critical to DNN efficiency~\cite{Eyeriss2016, yang2016systematic, gao2017tetris, gao2019tangram, DaDianNao2014, Ma2017dnnFPGA, Hegde2018morph, Mullapudi2016AutoHalide, yang2018dnn, whatmough2019vlsi, FusedCNN2016, lu2017flexflow, kwon2018maeri, whatmough2019fixy}. Orthogonal to generic data-reuse, we identify a new reuse dimension, inter-layer activation reuse (\texttt{ILAR}), that is uniquely enabled by our deconvolution transformation.
%, which translates a deconvolution layer to a set of convolution layers that share the same \textit{ifmap}.

%Many prior work have use some heuristic-base or exhaustive search to find the near-optimal solution~\cite{Mullapudi2016AutoHalide, yang2018dnn, Ma2017dnnFPGA}. Others proposed new approaches for dataflow scheduling along with their new memory systems based on the characteristics in memory access for some DNNs~\cite{Hegde2018morph, gao2017tetris}. 

%because of the additional reuse dimension, and our deconvolution transformation quadruples or even octuples the number of layers
Previous DNN mapping frameworks mostly rely on exhaustive search~\cite{yang2018dnn, yang2016systematic, Hegde2018morph}, which does not scale to exploiting \texttt{ILAR} (\Sect{sec:deconv:reuse}). 
Instead, \proj uses a constrained-optimization that can solved efficiently using dynamic programming. 
TETRIS~\cite{gao2017tetris} also uses a constrained-optimization for DNN scheduling, albeit with certain problem-specific simplifications. 
However, it does not exploit \texttt{ILAR}. Our formulation directly optimizes for latency rather than memory traffic~\cite{yang2016systematic, gao2017tetris} or resource utilization~\cite{Ma2017dnnFPGA}.

%leverages the particular compute pattern in deconvolution and propose constraint-solving based optimization along with its unique Inter-Layer Activation Reuse (ILAR), which explores the unique memory sharing across different sub-kernels. We formulate our deconvolution optimization as constraint problem and directly optimize the end-to-end latency instead of .










==> ASV_ Accelerated Stereo Vision System/sys.tex <==

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{system}
\caption{The \proj overview with augmentations shaded.}
\label{fig:system}
%\vspace{-10pt}
\end{figure}

\section{The ASV System}
\label{sec:sys}

Building on top of the ISM algorithm and the deconvolution optimizations, this section presents the software and hardware system of \proj.~\Fig{fig:system} gives a high-level system overview of \proj. We first present the software system (\Sect{sec:sys:sw}), and then discuss the architecture design decisions (\Sect{sec:sys:hw}).

\subsection{Software System}
\label{sec:sys:sw}

%\begin{algorithm}[t]
%\begin{algorithmic}
%\Function{MainRoutine}{$L, W$}
%	\State $Config \gets \{\}$
%    \For {$i \in $len(L)}
%    	\State $ l_i = L[i], w_i = W[i] $
%    	\If {$l_i = Conv$}
%      		\State $Config[l_i] \gets \Call{OptimizeConv}{l_i, w_i} $
%    	\Else
%        	\State $w_{sub} \gets \Call{SplitDeconv}{w_i} $
%      		\If {$\Call{Merge}{w_{sub}}$}
%        		\State $Config[l_i] \gets \Call{OptimizeDeconv}{l_i, w_{sub}} $
%    		\Else
%            	\State $Config[l_i] \gets \Call{OptimizeConv}{l_i, w_{sub}} $
%            \EndIf
%		\EndIf
%    \EndFor
%    \State \Return $Config$
%\EndFunction
%\end{algorithmic}
%\caption{Compiler Optimization Routine}
%\label{alg:main}
%\end{algorithm}

The goal of the software system in \proj is to map the ISM algorithm to the underlying hardware. 
The static mapping is done offline. 
There are three components in the ISM algorithm to map: stereo matching DNN, motion estimation, and local correspondence search. We rely on the user to supply a particular stereo DNN depending on their accuracy needs. Motion estimation and correspondence search are implemented using optical flow (OF) and block matching (BM), respectively, as described in \Sect{sec:algo:design}. We now describe how each component is processed by the software.

\paragraph{Mapping Stereo Matching DNN} For the deconvolution layer, the \proj software performs the deconvolution transformation, as well as the data reuse optimization. For convolution layers, while the deconvolution transformation does not apply, we apply the data reuse optimization \textit{without} ILAR. In the end, we obtain a transformed stereo DNN along with an execution schedule, which are both consumed by the hardware at runtime. The schedule includes the tiling strategy and buffer partitioning strategy for each layer.
%We do not claim new contributions in optimizations to the convolution layers, but still apply tiling optimizations to obtain a fairer baseline for comparison.

%The goal of the software system is to automatically map the operations in a DNN algorithm to a targeted hardware substrate. As we know, a DNN algorithm is often consisted of by a stack of operation layers with millions of computation operations. To find the optimal computation ordering seems time-consuming if not infeasible. To make this problem simpler, our compiler optimizes DNN algorithms in a layer-by-layer fashion. Within each layer, our optimization routine is able to reach a optimal configuration. Although, we are aware of some have studied fusing multiple layers and optimizing them all together~\cite{FusedCNN2016}, we are not considering this idea in our framework here. Still, our optimization routine can guarantee the optimal configuration in layer-by-layer fashion. Note that, we only map and optimize \texttt{Conv} and \texttt{Deconv} to the systolic array in our framework, the rest of operations are computationally negligible.

%The optimization routine proceeds as follows. For every single layer, it first converts non-\texttt{Conv} layers to \texttt{Conv} layers. Next, a unified routine is used to optimize \texttt{Conv} layers by using constraint optimization (more details in \Sect{subsec:dataflow_opti}). We elaborate how to convert a \texttt{Deconv} to a \texttt{Conv} with additional optimization on the utilization of the systolic array in \Sect{subsec:deconv_opti}. The pseudo code of our compiler optimization routine is shown in Algorithm~\ref{alg:main}.

\paragraph{Mapping OF/BM} The software maps the OF and BM algorithms in ISM to a set of convolution and/or activation operations that are directly interfaced with conventional DNN accelerators. The software translates the BM operation to a convolution layer (\Sect{sec:algo:design}), but calculating SAD instead of dot product at each window.

The OF computations include Gaussian blur, ``Compute Flow'' and ``Matrix Update'' operations (\mbox{\Sect{sec:algo:design}}), shown in the top-right box in~\mbox{\Fig{fig:system}}. Gaussian blur is naturally expressed as a convolution layer with one output channel. ``Compute Flow'' and ''Matrix Update'' are point-wise operations expressed as special activation functions.
%The rest of computations are replaced with a stub to indicate executions on hard-wired logics.

%In the end, the \proj software translates the entire ISM algorithm to a conventional convolution-like interface that gets loaded to the hardware.

%The \proj software generates a DNN like layer description for ME and CS, which gets loaded to the controller of the hardware along with the schedule of the DNN. Note that each Gaussian blur calculates, in classic DNN terms, one output channel, and therefore can only be expanded at one dimension on the systolic array, resulting in PE under-utilization. \fixme{maybe discuss in more detail what we mean by generating a schedule.}

\subsection{Hardware Architecture}
\label{sec:sys:hw}

Leveraging the software pass, the hardware requires only minimal, structured augmentations on top of a conventional DNN accelerator. We start from a baseline DNN accelerator and describe how the compute, memory, and control logic is augmented with \proj-specific architectural extensions.

\paragraph{Compute} Our baseline DNN accelerator consists of a TPU-like systolic PE array for convolution and a scalar unit for non-convolution operations, e.g., activation~\mbox{\cite{jouppi2017datacenter}}. Each PE consists of two 16-bit input registers, a 16-bit fixed-point MAC unit with a 32-bit accumulator register, and simple trivial control logic. This is identical to the PE in the TPU~\mbox{\cite{jouppi2017datacenter}}.

We use the systolic array as the baseline due to its efficiency in handling convolutions. However, our software optimizations do not depend on a particular baseline DNN architecture. Alternatives such as more flexible spatial architectures~\mbox{\cite{Eyeriss2016,chen2014diannao}} are also suitable, albeit requiring different constrained-optimization formulations to those presented in~\mbox{\Sect{sec:deconv:reuse}}. We will later demonstrate the effectiveness of our deconvolution optimizations on Eyeriss~\mbox{\cite{Eyeriss2016}}.

%We leave the comparison between different architectural choices for stereo vision to future work.
%the PE array not only executes the stereo DNNs for key frames, but also the Gaussian blur and BM operations for non-key frames. To support BM, 
\mbox{\proj} augments both the systolic array and the scalar unit in the baseline architecture to support the ISM algorithm. First, each PE is extended with the capability to accumulate absolute differences (i.e., $a \leftarrow a +|b - c|$) in addition to MAC in order to support BM. Second, we extend the scalar unit to support two additional point-wise operations: ``Compute Flow'' and ``Matrix Update''; both are required by OF (as illustrated in the bottom-right box in~\mbox{\Fig{fig:system}}).

Finally, the hardware includes a very small amount of additional logic to support the remaining operations in the ISM algorithm that are inefficient to map to either the systolic array or the point-wise scalar unit. 
These operations are comparisons and control-flow, and are orders of magnitude less costly in area and power compared to the systolic array and the scalar unit. 
For instance, BM requires comparing the SAD values across different matched blocks, and OF requires checking the value boundaries during "Matrix Update".

\paragraph{Memory} \proj uses the familiar three-level memory hierarchy~\cite{li2019mlmem}. Each PE has a small register file to exploit intra/inter-PE data reuse. A DMA engine coordinates data transfer between the on-chip global buffer and off-chip memory. The global buffer is temporally-shared between key frames and non-key frames. When processing key frames, the global buffer holds the ifmap, kernels, and ofmaps. The exact buffer partitioning is dictated by the \proj software.

When processing non-key frames, the global buffer holds four pieces of data: the pixels of the current and key frames, the Gaussian kernel, the motion vectors, and the disparity maps. The frame pixels dominate the storage requirement, but could be tiled because they are used in Gaussian blur and BM, both of which are convolution operations. The rest of the data cannot be tiled, and thus imposes a minimum buffer size. Assuming qHD resolution (960 $\times$ 540), we enforce a minimum buffer size of about 512 KB.

% motion vectors: 480*270*1*2 ~ 253 K
% disparity maps (new + old): 480*270*1*2 ~ 253 K
% Gaussian kernel: 15*15*2 ~ 0.4 K

\paragraph{Control} A micro-sequencer is used to coordinate the computation and memory accesses. In \proj, the sequencer also chooses key frames. Although complex adaptive schemes are feasible~\cite{zhu2018euphrates, buckler2018eva2}, we found that a simple strategy to statically set the key-frame window suffices (\Sect{sec:eval:ac}).

%The sequencer reads the schedule passed down by the software to coordinate the computations and the memory accesses. We implement the controller through a micro-code store rather than hard-wired logics to accommodate different schedules optimized for different hardware capabilities.
%Programmable micro-controllers (e.g., ARM Cortex-M4~\cite{??}) would enable more flexibilities, but they typically run at low frequencies that do not keep up with the compute datapath.

%\Fig{fig:layout} shows the schematic layout of our hardware design. In our design, we use a double on-chip buffer to parallelize the compute stage of current on-chip data with the load/store stage of next round. To compute the \textit{ofmap}, the memory controller will signal systolic array to load corresponding weights and \textit{ifmap} from the on-chip buffer. After computation of \textit{ofmap}, the output from the systolic array will go through a reduction unit if necessary before being stored back to the on-chip buffer. Meanwhile, to cope with the deconvolution operation, the memory controller will occasionally signal the systolic array to load/store the intermediate results into a proper register. Next, we will introduce each components in details.




==> disc.tex <==
\section{Discussion}
% What can I put in here?


==> overview.tex <==

\begin{figure*}
\centering
\begin{minipage}{.4\textwidth}
  \centering
  \includegraphics[width=\linewidth]{overview}
  \captionof{figure}{Overview of our framework.}
  \label{fig:overview}
\end{minipage}%
\begin{minipage}{.6\textwidth}
  \centering
  \includegraphics[width=\linewidth]{motion_algorithm}
  \captionof{figure}{Comparison of DNN pipeline with our integrated pipeline.}
  \label{fig:motion_algorithm}
\end{minipage}
\end{figure*}

\section{System Overview}

As we shown in \Sect{subsec:tradeoff}, it is necessary to design a stereo vision framework that supports a range of stereo vision algorithms. Meanwhile, to achieve the global optimal in the design space, we co-design algorithm and hardware to fully explore the unique characteristics of stereo vision. Here, we overview our design in three dimensions: algorithm, compiler and hardware, and explain how each component collaborate with others. 

\Fig{fig:overview} shows the stack of our design. At the top of our stack, a stereo vision runtime serves as an interface to varying stereo vision applications. To support different DNN algorithms, we design our stereo vision runtime that can embed any stereo vision applications with our integrated algorithms. At the bottom of our stack, we designed our stereo engine to support any computations in both classic and DNN algorithms in stereo vision pipelines. The key to bridge the runtime and the hardware is our compiler. Our compiler can automatically map any operation in algorithms onto the hardware. Meanwhile, our compiler optimizes the dataflow of stereo vision program and the hardware configuration to a global optimal under some constraints of hardware recourse. Next, we shortly highlight key features of each components in our framework, more details are in later sections.

\paragraph{Integrated Algorithm} As we have shown in \Sect{subsec:tradeoff}, on one hand, the state-of-the-art DNN algorithms are accurate but computationally expensive for most commodity devices, on the other hand, conventional algorithms are faster but poor in accuracy. In order to reduce the latency of DNN algorithms, we propose a runtime algorithm that couples DNN algorithms with the idea, triangulation, from conventional algorithms. By combining the merits of both, our runtime can achieve a substantial improvement on runtime performance and energy saving without substantial accuracy loss.

\paragraph{Hardware Support} To support varying operations in both conventional and DNN algorithms, we modify the classic design of systolic array. The modified systolic array can support all the key operations in both algorithms. We want a unified hardware instead of one hardware for each algorithm or operation. In addition, we design a memory controller to help with managing the dataflow on and off the chip. The overall design lets us avoid separate IP blocks per operation and some redundant computations, such as in \texttt{Deconv}. Previous studies have proposed special IP blocks to avoid the computational redundancy in \texttt{Deconv}~\cite{song2018GAN, Yazdanbakhsh2018GAN}. However, additional hardware for \texttt{Deconv} is hardly acceptable, especially on mobile platforms.

\paragraph{Compiler Optimization} 
In our design, the compiler has two key features. First, it can map the key operations in stereo vision algorithms to the modified systolic array. Second, our compiler conducts an unique dataflow optimization using constraint optimization. Doing this transformation, our compiler can use off-the-shelf solvers to configure the optimal dataflow for a particular hardware.




==> plan.tex <==
\section{Outline}
\begin{itemize}
\item Background 
\begin{enumerate}
\item Stereo vision: introduce two parts: the general procedure of stereo matching, and triangulation to compute depth map from disparity map.
\item CNN: introduce general CNN convolution and address 3D CNN in some stereo matching DNN. Last, introduce deconvolution layer.
\end{enumerate}

\item Motivation: show the trade-off between computation and performance. Different use scenarios need to use different DNN based on DNNs latency and accuracy.

\item{Optimization}
\begin{enumerate}
\item Dataflow optimization: by changing the dataflow, the total latency of entire computation can be dramatically reduced. We propose two type of dataflow optimization comparing to previous studies. 
\begin{itemize}
\item First, we based on a typical CNN, we propose a algorithm pipeline to accelerate the entire CNN computation. 
\item Second, based on the unique character of deconvolution, we propose a new way to compute with a HW support.
\end{itemize}

\item Algorithm-level optimization: Further exploring the trade-offs between accuracy and performance, we leverage two unique characteristics on stereo vision.
\begin{itemize}
\item Use triangulation to leverage the result from the previous frames and reduce the computation cost of DNN.
\item Most of stereo matching DNN pipeline, in their deconvolution stage, will compute a small-scale result and fine-tune it at later stages. We take advantage of this characteristics and use simple extrapolation to compute fine-grained result.
\end{itemize}

\end{enumerate}  % optimization



\item Hardware support 
\begin{enumerate}
\item Modification on systolic array: to have 4 registers per MAC unit and a signal controller to signal which register should store the current computed value.
\item Buffer controller: control the partition of buffer lane and load/store of each buffer lane.
\end{enumerate}

\end{itemize}
















